VStore: A Data Store for Analytics on Large Videos

We present VStore, a data store for supporting fast, resource-efficient analytics over large archival videos. VStore manages video ingestion, storage, retrieval, and consumption. It controls video formats along the video data path. It is challenged by i) the huge combinatorial space of video format knobs; ii) the complex impacts of these knobs and their high profiling cost; iii) optimizing for multiple resource types. It explores an idea called backward derivation of configuration: in the opposite direction along the video data path, VStore passes the video quantity and quality expected by analytics backward to retrieval, to storage, and to ingestion. In this process, VStore derives an optimal set of video formats, optimizing for different resources in a progressive manner. VStore automatically derives large, complex configurations consisting of more than one hundred knobs over tens of video formats. In response to queries, VStore selects video formats catering to the executed operators and the target accuracy. It streams video data from disks through decoder to operators. It runs queries as fast as 362x of video realtime.

==> eval-model.tex <==
% !TeX root = main.tex

\section{Model Evaluation and Discussions}
\label{sec:eval}

The model evaluation answers the following questions:

\begin{description}[align=left]
	\item [\S\ref{sec:accuracy}] Does our cost model accurately estimate the actual performance?
	\item [\S\ref{sec:offline}] Can our tool/model suggest cost-effective hardware planning?	
\end{description}

\subsection{Model Accuracy}
\label{sec:accuracy}
We will first evaluate the accuracy of our cost model. \note{Upon the accurate model, the following discussion regarding the optimization and end-to-end performance are valid.}
We pick 5 typical configurations with different storage capacities and decoding abilities.

From figure~\ref{fig:accuracy}, our cost model has at most XX\% difference compared with the actual performance.

\input{fig-model-accuracy}

\subsection{Offline Model Supports}
\label{sec:offline}
Upon the current optimal configuration, \sys{} will provide possible configurations that the user can take into consideration in the future, either new storage devices or a more powerful GPU.
\subsubsection{Hardware Planning}


It produces a plot of cost-performance trade-offs as shown in \note{Figure. xxx}. 
On this plot, each point represents a hardware setup. 
The X-axis shows the monetary costs of hardware setups and the Y-axis shows the best query performance of a hardware setup (with the optimal \istream{} configuration given by the solver). 

ii) look for Pareto optimal points ... 

\note{need a figure, showing all the points and the frontier}

The planner identifies and presents to the user all the points on the Pareto frontier, 
defined as \note{add formal def from somewhere else}. 
Intuitively, each point represents the hardware setup that gives best the performance at the same cost point;
any other setup either has higher cost or lower performance. 
Hence, the user only has to consider these points in trading off between performance and hardware cost. 
\note{How does the planner identify the frontier? Todo: revisit videostorm and learn}

%and the configuration on this line are promised to be the most cost-efficiency configuration under the same budget. 
%Dots on the right hand side of the frontier are not recommended to the user, because the user can always a the higher or same performance with less configuration cost by shifting left to the Pareto optimal. 
%Furthermore, two constraints of the configuration choice will be the hardware cost budget and the limit of CV output.
%The map will only show the possible configuration in the region restricted by the vertical line (budget limit) and the horizontal line (demand for highest performance). 

With the planner, we will show what-if analysis in the face of hardware trends (e.g. lower decoder throughput per dollar) in \sect{eval}.

%The evaluation of hardware planning goes to \note{section 9}.
%\note{Provide insights from hardware planning} impact of weights, 
%1. The distribution of cluster (related to decoder number, but the boundary melts down when the weights are closer)
%2. Discuss the frontier trend, and the Pareto optimal on the frontier --
%Equal weights(extreme case), prefer hot data (0.9,0.09,0.01)


\paragraph{Pareto Frontier}
The lines in figure XXX represents combinations of different weights of data temperatures regarding the Pareto Frontier, the trend of optimal configuration under different costs. 
The graph shows that it takes small amount of investment from deficit configurations to decent configurations to boost the performance; while the resources already satisfy most of the data demands, the user will need to invest more hardware to get a little improvements in throughput. 

\paragraph{General Insights}
We can draw useful conclusions from the following general conditions.
\begin{itemize}
	\item \textbf{Different weights on data temperature} 
	
	As shown in Figure~\ref{fig:hw_plan1} the weights on different data temperatures can have a large impact on the trend of Pareto Frontier.
	Normally, the amount of video data ranks as ascending order of hot, warm and cold.
	If more recent data is more interesting and would likely to be visited more, which means higher weights are on hot or warm data, less storage space is needed to achieve high throughput. 
	So under the same configuration cost, (0.9, 0.09, 0.01) out performs the other two weight distributions like (0.7, 0.2, 0.1) and (0.34, 0.33, 0.33).
	\item \textbf{Different data sources}
	
	As shown in Figure~\ref{fig:hw_plan2}, due to the high variance of video data, the probability of activating each stage also have a large difference.
	Normally, earlier stages are often equipped with lower resolution data and faster CV operators; later stages are often fed by higher resolution frames and slower CV operators, and retard the whole pipeline performance.
\end{itemize}

\paragraph{Provision for future}
	\note{use some real hardware numbers, e.g. mobile GPU with many decoders. actual SSD. non-volatile memory}
	
Since decoders and the storage devices are becoming cheaper in the future, we also consider these scenarios.
Following Narayanan \emph{et al.}~\cite{narayanan09eurosys}, we also have the definition of performance/dollar (fps/\$) ratio for decoders.
\begin{itemize}  
	\item \textbf{Decoders}  \note{not GPU, but decoders}
	\begin{itemize}
		\item \textbf{Cheaper decoders}
	
		As shown in Figure~\ref{fig:hw_plan3}, by cutting the monetary cost in our cost model provided in \note{section XXX}, we find out that the Pareto frontier shifts left, and some of the optimal points are replaced.
		However, the performance still converges to the same number.
	
		\item \textbf{Mobile GPU with many decoders}
	\end{itemize}
\end{itemize}
For storage devices, we have another two metrics including Read/Write speed/dollar (speed/\$, or $S_A$) and capacity/dollar (GB/\$, or $G_B$). 
If we consider the break-even point~\cite{narayanan09eurosys} between two storages, workloads with Speed/GB higher than $S_A$/$G_B$ are better served on storage B.
\begin{itemize}  
\item \textbf{Storage Devices}
	\begin{itemize}
		\item \textbf{NVME instead of SSD}
		\item \textbf{Faster SSD at the same price}
	
		As shown in Figure~\ref{fig:hw_plan4}, faster SSD with the same cost yields to higher performance. 
	\end{itemize}
\end{itemize}

Besides, sometimes the budget is not affordable for the administrator to manage an enterprise machine, so we compare the cost-efficiency between server level and desktop level 
\begin{itemize}
	\item \textbf{Consumer SSD vs. Enterprise SSD}
	\item \textbf{RAID HDD Arrays  vs. Single HDD}
	\item \textbf{...}
\end{itemize}
\input{fig-hwplanning}

\subsubsection{Reconfiguration and Data Migration}
\sys{} reconfigures the i-stream in order to meet the throughput requirements of CV algorithms as soon as possible.
In this case, the order of different migration tasks have different impact on the immediate change on performance. 
The evaluation regarding the migration cost is in section \S\ref{sec:migration}.

==> eval.tex <==
% !TeX root = main.tex

\section{Evaluation}
\label{sec:eval}

\note{draft this -- what questions have to be answered}
We carried out evaluations of our system on two known deep learning frameworks -- NoScope~\cite{noscope} and license plate reader (OpenALPR~\cite{openalpr}).
\paragraph{License Plate Recognition}

OpenALPR car plate recognition pipeline is roughly divided into three stages. 
First, a motion detector will identify moving objects between continuous frames. 
If no motion detected, it will skip the upcoming stages. 
Normally, the motion detection can boost to 10k on 180p videos. 
Second, if motion is detected, the program will give a list of ROIs that might contain license plates.
This is the most expensive operator in the whole pipeline, and usually 720p frames are needed.
Third, alpr will perform recognition on each of the ROI by characterization and OCR.

\paragraph{NoScope}

NoScope supports 1000x faster deep learning queries by harnessing the temporal/spatial locality over videos, dramatically reduces the computation on each frame.
The specialized model and difference detector boosts the processing speed to more than 10K fps.

The evaluation answers the following questions:

\begin{description}[align=left]
	\item [\S\ref{sec:accuracy}] Does our cost model accurately estimate the actual performance?
	\item [\S\ref{sec:offline}] Can our tool/model suggest cost-effective hardware planning?	
	\item [\S\ref{sec:insertion}] Is the insertion overhead of \sys{} affordable when ingesting multiple video streams.
	build of istream. (has little to do with the model per se). 
	\item [\S\ref{sec:perf}] Does \sys{} provide the best end-to-end query performance?
	%end to end performance. do we have good performance? how does our istream solution (from solver) contribute to good performance, etc? -- based on experiments. 
	\item [\S\ref{fig:migration}]Migration: does migration mechanism ....?
%	\item [\S\ref{sec:online}] How does \sys{} dynamically support online operations?
\end{description}

\subsection{Performance--Cost Accuracy}
\label{sec:accuracy}
We will first evaluate the accuracy of our cost model. \note{Upon the accurate model, the following discussion regarding the optimization and end-to-end performance are valid.}
We pick 5 typical configurations with different storage capacities and decoding abilities.

From figure XXX, our cost model has at most XX\% difference compared with the actual performance.

\input{fig-model-accuracy}

\subsection{Offline Decisions}
\label{sec:offline}
\sys{} takes two stages to guide the i-stream configuration -- optimal configuration and hardware planning. 
First, the user provide the current hardware configuration, and \sys{} will give the user the optimal i-stream configuration under the current condition. 
Second, \sys{} will provide possible configurations that the user can take into consideration in the future, either new storage devices or a more powerful GPU.
\subsubsection{Hardware Planning}
\paragraph{Pareto Frontier}
The lines in figure XXX represents combinations of different weights of data temperatures regarding the Pareto Frontier, the trend of optimal configuration under different costs. 
The graph shows that it takes small amount of investment from deficit configurations to decent configurations to boost the performance; while the resources already satisfy most of the data demands, the user will need to invest more hardware to get a little improvements in throughput. 

\paragraph{General Insights}
We can draw useful conclusions from the following general conditions.
\begin{itemize}
	\item \textbf{Different weights on data temperature} 
	The weights on different data temperatures can have a large impact on the trend of Pareto Frontier.
	Normally, the amount of video data ranks as ascending order of hot, warm and cold.
	If more recent data is more interesting and would likely to be visited more, which means higher weights are on hot or warm data, less storage space is needed to achieve high throughput. 
	So under the same configuration cost, (0.9, 0.09, 0.01) out performs the other two weight distributions like (0.7, 0.2, 0.1) and (0.34, 0.33, 0.33).
	\item \textbf{Different data sources}
	Due to the high variance of video data, the probability of activating each stage also have a large difference.
	Normally, earlier stages are often equipped with lower resolution data and faster CV operators; later stages are often fed by higher resolution frames and slower CV operators, and retard the whole pipeline performance.

\end{itemize}

\paragraph{Provision for future}
Since GPUs and the storage devices are becoming cheaper in the future, we also consider these scenarios.
\begin{itemize}
	\item \textbf{GPU becomes cheaper} 
	By cutting the monetary cost in our cost model provided in \note{section XXX}, we find out that the Pareto frontier shifts left, and some of the optimal points are replaced.
	However, the performance still converges to the same number.
	\item \textbf{Storage becomes faster at the same price}

\end{itemize}

\input{fig-hwplanning}

\subsubsection{Reconfiguration and Data Migration}
\sys{} reconfigures the i-stream in order to meet the throughput requirements of CV algorithms as soon as possible.
In this case, the order of different migration tasks have different impact on the immediate change on performance. 
The evaluation regarding the migration cost is in section \S\ref{sec:online}.

\subsection{Insertion}
\label{sec:insertion}

\sys{} is implemented but not restricted to software decoding. 
The total insertion speed is xxx fps.
Assume the ingested video stream is 30fps, \sys{} can support up to xxx video stream.

\input{fig-insertion}

\subsection{Online Supports}
\label{sec:online}
\subsubsection{Query Performance}
One primary goal of \sys{} is to mitigate the limitation of disk bandwidth on performance by exploiting i-stream configurations on heterogeneous storage tiers. 
We carried out evaluations of our system on two known deep learning frameworks.
In the graph, we compare the disk utilization and the performance with known numbers provided from state-of-the-art frameworks.
Note that in NoScope~\cite{noscope}, all the decoded frames are kept in memory, instead of the end-to-end streaming case that we provided.
All measurements are carried out by a cold cache.

\input{fig-query-performance}

\paragraph{Scheduler}
In order to make the pipeline smooth, we provide the scheduler that keeps track of different tasks and map each task to different cores/threads.
Since each operator have different requirement on i-stream configurations, each of them proceed at different pace.
The operator's presence avoids the unbalanced situation where some operators starve and some of them run too early ahead of time.

\textbf{scale to the number of ops? number of accuracy levels?}

\paragraph{Data/Decoding Scalability}
\note{the graph/paragraph can be cut}
We exploit parallelism on many of the CPU-intensive operations over multiple cores by using OpenMP.
However, it would be less efficiency to flood to as many cores as we can.
Through our experiments on a 56-core machine, 30 threads parallelism is the best choice, and if we use more cores, the performance will be even worse due to hardware contention. \note{needs verification}.
From the profiling results of Intel VTune, the CPI rate stays identical when the number of cores are under 35.
However, when we further exploiting parallelism onto more cores, the CPI rate will increase, which indicates that the scalability actually goes down.
Other system utilization results like average memory bandwidth and memory bound rate both increase nearly linearly with the number of cores.

Decoding also benefits from parallelism. 
In the evaluation phase, we run the decoders on a CPU-only machine, however, in \sys{}, the decoding is not restricted to CPUs.
From the graph, we noticed that the decoding performance saturates at XXX cores.

\paragraph{Trade-offs between storage space and performance}
\note{Compare the extra storage usage (compared to one resolution) vs performance gain}

\subsubsection{Runtime Migration}
We track the performance between each migration tasks carried out in sequence by \sys{}, and compare to arbitrary random sequences of migration tasks.
Our approach approaches the higher resolution faster than other arbitrary approaches.
\input{fig-migration}



==> fig-arch.tex <==
% !TeX root = main.tex

\begin{figure}[t!]
\centering
\includegraphics[width=0.45\textwidth{}]{./figs/arch} 
%\vspace{-10pt}		% use as needed
\caption{The \sys{} architecture}
\label{fig:arch}
%\vspace{-20pt}		% use as needed
\end{figure}


==> fig-cascade.tex <==
% !TeX root = main.tex

\begin{figure}[t!]
\centering
\includegraphics[width=0.45\textwidth{}]{./figs/cascade} 
%\missingfigure[figwidth=6cm]{Kernel support}
%\vspace{-10pt}		% use as needed
\caption{A cascade of operators in one sample CV analytics. Each operator demands different fidelities and exhibits varying throughputs XXX: show ALPR measurement XXXX}
\label{fig:cascade}

%\vspace{-20pt}		% use as needed
\end{figure}


==> fig-hwplanning.tex <==
% !TeX root = main.tex

\begin{figure*}[t!]
	
	\captionsetup[subfigure]{labelformat=empty,justification=centering} % xzl
	%\quad \quad \quad
	\centering				
	\begin{minipage}[b]{0.4\textwidth}
		\includegraphics[width=1\textwidth]{figs/fig1.pdf}
		\subcaption{(a) \textbf{Different weights on temperatures}}
		\label{fig:hw_plan1}
	\end{minipage}
	~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
	%(or a blank line to force the subfigure onto a new line)
	\begin{minipage}[b]{0.4\textwidth}
		\includegraphics[width=1\textwidth]{figs/fig2.pdf}
		\subcaption{(b) \textbf{Different videos}}
		\label{fig:hw_plan2}
	\end{minipage}
	 %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
	%(or a blank line to force the subfigure onto a new line)
	
	\centering				
	\begin{minipage}[b]{0.4\textwidth}
		\includegraphics[width=1\textwidth]{figs/fig3.pdf}
		\subcaption{(c) \textbf{Cheaper GPU}}
		\label{fig:hw_plan3}
	\end{minipage}
	~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
	%(or a blank line to force the subfigure onto a new line)
	\begin{minipage}[b]{0.4\textwidth}
		\includegraphics[width=1\textwidth]{figs/fig4.pdf}
		\subcaption{(d) \textbf{Faster SSD}}
		\label{fig:hw_plan4}
	\end{minipage}
	\vspace{20pt}
	\caption{Hardware Planning}
\end{figure*}

==> fig-insertion.tex <==
% !TeX root = main.tex

\begin{figure}[t!]
	
	%\captionsetup[subfigure]{labelformat=empty,justification=centering} % xzl
	%\quad \quad \quad
	%\centering				
	\begin{minipage}[b]{0.4\textwidth}
		\includegraphics[width=1\textwidth]{figs/insertion-cases}
		\subcaption{\textbf{Different Insertion Cases}}

	\end{minipage}
	%~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
	%(or a blank line to force the subfigure onto a new line)
	%\hfill
	\begin{minipage}[b]{0.4\textwidth}
		\includegraphics[width=1\textwidth]{figs/fig-insertion}
		\subcaption{\textbf{Max Incoming Streams Supported}}

	\end{minipage}
	\vspace{10pt}
	\caption{Insertion Performance}
	\label{fig:insertion}
\end{figure}

==> fig-istream-store.tex <==
% !TeX root = main.tex

\begin{figure}[t!]
\centering
\includegraphics[width=0.45\textwidth{}]{./figs/istream-store} 
%\vspace{-10pt}		% use as needed
\caption{Storage format of istreams}
\label{fig:istream-store}
%\vspace{-20pt}		% use as needed
\end{figure}


==> fig-merge.tex <==
% !TeX root = main.tex

\begin{figure}[t!]
\centering
   
  		
	\begin{subfigure}[b]{0.5\textwidth}
   \includegraphics[width=1\linewidth]{figs/plot/eval-merge/eval-merge.pdf}
%   \caption{bla bla bla}
	\vspace{2mm}
%   \label{fig:concept:1} 
	\end{subfigure}
	
%	\begin{subfigure}[b]{0.45\textwidth}
%	   \includegraphics[width=1\linewidth]{figs/concept-2}
%	   \caption{Parallel operator execution. Engine batches records in bundles, consuming and producing bundles in multiple windows in parallel
%	   }
%%	\label{fig:concept:op} 
%	\end{subfigure}

\caption{(a) Merge time comparison, with 12 FCs. (b) show results for 24 \FC{}s as well XXX more videos? Merging all FC takes 475 profiling (10s video) in 1 minute}

\vspace{-10pt}		% use as needed

\label{fig:merge}
\end{figure}

==> fig-migration.tex <==
% !TeX root = main.tex

\begin{figure}[t!]
	\centering
	\includegraphics[width=0.45\textwidth{}]{./figs/migration} 
	%\missingfigure[figwidth=6cm]{Workflow}
	\vspace{10pt}		% use as needed
	\caption{Query Performance Under Video Data Migration }
	\label{fig:migration}
	\vspace{0pt}		% use as needed
\end{figure}


==> fig-model-accuracy.tex <==
% !TeX root = main.tex

\begin{figure}[t!]
\centering
%\includegraphics[width=0.45\textwidth{}]{./figs/benchmarks} 
\includegraphics[width=0.45\textwidth{}]{./figs/model-accuracy} 
\vspace{10pt}		% use as needed
\caption{Model Accuracy}
\label{fig:accuracy}
\vspace{0pt}		% use as needed
\end{figure}


==> fig-query-performance.tex <==
% !TeX root = main.tex

\begin{figure}[t!]
	\centering
	\includegraphics[width=0.45\textwidth{}]{./figs/query-perf} 
	%\missingfigure[figwidth=6cm]{Workflow}
	\vspace{10pt}		% use as needed
	\caption{Query Performance Under Different Configurations}
	\label{fig:perf}
	\vspace{0pt}		% use as needed
\end{figure}


==> fig-sample-minipage.tex <==
% !TeX root = main.tex

\begin{figure}[!t]

	\begin{minipage}[b]{0.23\textwidth}
		\includegraphics[width=1\textwidth]{figs/plot/fair/cpu/cpu}
		        \subcaption{CPU}
		\label{fig:gull}
	\end{minipage}
	~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
	%(or a blank line to force the subfigure onto a new line)
	\begin{minipage}[b]{0.23\textwidth}
		%		\includegraphics[width=\textwidth]{figs/plot/scalability/wingrep.pdf}
		\includegraphics[width=1\textwidth]{figs/plot/fair/dsp/dsp}
		        \subcaption{DSP}
		\label{fig:tiger}
	\end{minipage}	

	\begin{minipage}[b]{0.23\textwidth}
		%		\includegraphics[width=\textwidth]{figs/plot/scalability/wingrep.pdf}
		\includegraphics[width=1\textwidth]{figs/plot/fair/gpu/gpu}
		        \subcaption{GPU}
		\label{fig:tiger}
	\end{minipage}	
	~
	\begin{minipage}[b]{0.23\textwidth}
	%		\includegraphics[width=\textwidth]{figs/plot/scalability/wingrep.pdf}
	\includegraphics[width=1\textwidth]{figs/plot/fair/wifi/wifi}
	        \subcaption{WiFi}
	\label{fig:tiger}
	\end{minipage}	
		
	\caption{Throughputs of co-running app instances, before and after one instance (marked with *) enters \psbox{}. 
%	\psbox{} ensures fairness by keeping throughputs of other apps largely unchanged.
	}
%	\vspace{-10pt}		% use as needed
	\label{fig:fair}
\end{figure}

==> fig-sample-multi.tex <==
% !TeX root = main.tex

\begin{figure*}

	\captionsetup[subfigure]{labelformat=empty,justification=centering} % xzl
	
	\quad \quad \quad
	\begin{minipage}[b]{0.9\textwidth}
		\includegraphics[width=1\textwidth]{figs/power-top}
	\end{minipage}
	~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
%	\centering					
	\begin{minipage}[b]{0.03\textwidth}	
		\begin{picture}(0.01,10)
		  \put(0.01,50){\rotatebox{90}{CPU}}
		\end{picture}
	\end{minipage}	
	~			
	\centering				
	\begin{minipage}[b]{0.18\textwidth}
		\includegraphics[width=1\textwidth]{figs/plot/power/cpu/calib_alone.pdf}
		\subcaption{\textbf{calib3d} \\ 936mJ}
%		\label{fig:tiger}
	\end{minipage}
	~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
	%(or a blank line to force the subfigure onto a new line)
	\begin{minipage}[b]{0.18\textwidth}
		\includegraphics[width=1\textwidth]{figs/plot/power/cpu/calibX+body.pdf}
		\subcaption{\textbf{calib3d} [w/ body] \\ 922mJ (-1.5\%)}
	\end{minipage}
	~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
	%(or a blank line to force the subfigure onto a new line)
	\begin{minipage}[b]{0.18\textwidth}
		\includegraphics[width=1\textwidth]{figs/plot/power/cpu/calibX+dedup.pdf}
		\subcaption{\textbf{calib3d} [w/ dedup] \\ 925mJ (-1.2\%)}
%		\label{fig:mouse}
	\end{minipage}
	~
	\begin{minipage}[b]{0.18\textwidth}
		\includegraphics[width=1\textwidth]{figs/plot/power/cpu/calib+body.pdf}
		\subcaption{\textbf{calib3d} [w/ body] \\ 853mJ (-8.9\%)}
%		\label{fig:mouse}
	\end{minipage}    
	~
	\begin{minipage}[b]{0.18\textwidth}
		\includegraphics[width=1\textwidth]{figs/plot/power/cpu/calib+dedup.pdf}
		\subcaption{\textbf{calib3d} [w/ dedup] \\ 804mJ (-14.1\%)}
%		\label{fig:mouse}
	\end{minipage}    	
	~
	\begin{minipage}[b]{0.03\textwidth}	
		\begin{picture}(0.01,10)
		  \put(0.01,50){\rotatebox{90}{DSP}}
		\end{picture}
	\end{minipage}	
	~		
    \centering
    \begin{minipage}[b]{0.18\textwidth}
        \includegraphics[width=1\textwidth]{figs/plot/power/dsp/dgemm_alone.pdf}
%        \caption{wingrep \makalu{}}
		\subcaption{\textbf{dgemm} \\ 3018mJ }
        \label{fig:gull}
    \end{minipage}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
    \begin{minipage}[b]{0.18\textwidth}
%		\includegraphics[width=\textwidth]{figs/plot/scalability/wingrep.pdf}
		\includegraphics[width=1\textwidth]{figs/plot/power/dsp/dgemmX+sgemm.pdf}
		\subcaption{\textbf{dgemm} [w/ sgemm] \\ 2906mJ (-3.7\%)}
        \label{fig:tiger}
    \end{minipage}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    %(or a blank line to force the subfigure onto a new line)
    \begin{minipage}[b]{0.18\textwidth}
        \includegraphics[width=1\textwidth]{figs/plot/power/dsp/dgemmX+monte+sgemm.pdf}
		\subcaption{\textbf{dgemm}[w/monte+sgemm] \\ 2959mJ (-2.0\%)}
%        \label{fig:mouse}
    \end{minipage}
    ~
    \begin{minipage}[b]{0.18\textwidth}
        \includegraphics[width=1\textwidth]{figs/plot/power/dsp/dgemm+sgemm.pdf}
		\subcaption{\textbf{dgemm} [w/ sgemm] \\ 1560mJ (-48.3\%)}
%        \label{fig:mouse}
    \end{minipage}    
	~
    \begin{minipage}[b]{0.18\textwidth}
        \includegraphics[width=1\textwidth]{figs/plot/power/dsp/dgemm+monte+sgemm.pdf}
		\subcaption{\textbf{dgemm}[w/monte+sgemm] \\ 1110mJ (-63.2\%)}
        \label{fig:mouse}
    \end{minipage}    
%    \vspace{-10pt}		% use as needed
	~
	\begin{minipage}[b]{0.03\textwidth}	
		\begin{picture}(0.01,10)
		  \put(0.01,50){\rotatebox{90}{GPU}}
		\end{picture}
	\end{minipage}	
	~	
	\centering
	\begin{minipage}[b]{0.18\textwidth}
		\includegraphics[width=1\textwidth]{figs/plot/power/pvr/browser_alone.pdf}
		\subcaption{\textbf{browser} \\ 201mJ}
	\end{minipage}
	~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
	%(or a blank line to force the subfigure onto a new line)
	\begin{minipage}[b]{0.18\textwidth}
		%		\includegraphics[width=\textwidth]{figs/plot/scalability/wingrep.pdf}
		\includegraphics[width=1\textwidth]{figs/plot/power/pvr/browserX+magic.pdf}
		\subcaption{\textbf{browser} [w/ magic] \\ 199mJ (-0.9\%)}
	\end{minipage}
	~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
	%(or a blank line to force the subfigure onto a new line)
	\begin{minipage}[b]{0.18\textwidth}
		\includegraphics[width=1\textwidth]{figs/plot/power/pvr/browserX+tri.pdf}
		\subcaption{\textbf{browser} [w/ triangle] \\ 201mJ (0\%)}
	\end{minipage}
	~
	\begin{minipage}[b]{0.18\textwidth}
		\includegraphics[width=1\textwidth]{figs/plot/power/pvr/browser+magic.pdf}
		\subcaption{\textbf{browser} [w/ magic] \\ 211mJ (+5.0\%)}
	\end{minipage}    
	~
	\begin{minipage}[b]{0.18\textwidth}
		\includegraphics[width=1\textwidth]{figs/plot/power/pvr/browser+tri.pdf}
		\subcaption{\textbf{browser} [w/ triangle] \\ 172mJ (-14.4\%)}
	\end{minipage}    
	~
	\begin{minipage}[b]{0.03\textwidth}	
		\begin{picture}(0.01,10)
		  \put(0.01,50){\rotatebox{90}{WiFi}}
		\end{picture}
	\end{minipage}	
	~	
	\centering
	\begin{minipage}[b]{0.18\textwidth}
		\includegraphics[width=1\textwidth]{figs/plot/power/wifi/links_alone.pdf}
		\subcaption{\textbf{browser} \\ 267mJ}
	\end{minipage}
	~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
	%(or a blank line to force the subfigure onto a new line)
	\begin{minipage}[b]{0.18\textwidth}
		\includegraphics[width=1\textwidth]{figs/plot/power/wifi/linksX+scp.pdf}
		\subcaption{\textbf{browser} [w/ scp]\\ 273mJ (+2.2\%)}
	\end{minipage}
	~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
	%(or a blank line to force the subfigure onto a new line)
	\begin{minipage}[b]{0.18\textwidth}
		\includegraphics[width=1\textwidth]{figs/plot/power/wifi/linksX+wget.pdf}
		\subcaption{\textbf{browser} [w/ wget] \\ 313mJ (+17.2\%)}
	\end{minipage}
	~
	\begin{minipage}[b]{0.18\textwidth}
		\includegraphics[width=1\textwidth]{figs/plot/power/wifi/links+scp.pdf}
		\subcaption{\textbf{browser} [w/ scp] \\ 412mJ (+35.2\%)}
	\end{minipage}    
	~
	\begin{minipage}[b]{0.18\textwidth}
		\includegraphics[width=1\textwidth]{figs/plot/power/wifi/links+wget.pdf}
		\subcaption{\textbf{browser} [w/ wget] \\ 455mJ (+41.3\%)}
	\end{minipage}    
	
	\caption{\textbf{Power of the benchmark scenarios}. In all plots, x-axis: Time/Sec; y-axis: Power/Watt.
%		Each row shows a set of scenarios that test a particular driver.
%		Each row corresponds to the results of a particular driver.
%		Column 1: one app runs alone; 
%		Column 2 -- 5: the app co-runs with other apps. 
		In each row: even as an app co-runs with different apps (column 2--5), \psbox{} provides it with consistent power observations (column 2 \& 3), which are close to the power of the app running alone (column 1).
		This contrasts to the power attributed to the app by an existing accounting approach (column 4 \& 5).
		The numbers under each plot show the app's total energy and the difference compared to the energy when the app runs alone.
		Some plots cannot display full length of power activities due to space limit.
		}
	\label{fig:power}
	\vspace{-10pt}
\end{figure*}


==> fig-sample-single.tex <==
% !TeX root = main.tex

\begin{figure}[t!]
\centering
%\includegraphics[width=0.45\textwidth{}]{./figs/benchmarks} 
\missingfigure[figwidth=6cm]{Kernel support}
\vspace{-10pt}		% use as needed
\caption{This is the caption figure}
\label{tab:benchmarks}
\vspace{-20pt}		% use as needed
\end{figure}


==> fig-sample-subfigure.tex <==
% !TeX root = main.tex

\begin{figure}[t!]
\centering
   \begin{subfigure}[b]{0.4\textwidth}
   \includegraphics[width=1\linewidth]{figs/plot/motiv/spatial/both4/power}
   \caption{Total CPU power of two co-running process instances, one on each core, compared to 2$\times$ power of one instance running alone. Hardware: 2$\times$core Cortex-A15}
   % Benchmark: cpp drawing tutorial 1
	\vspace{2mm}
   \label{fig:motiv:spatial} 
	\end{subfigure}
% /home/xzl/Dropbox/private/drafts/powersandbox/results/motiv/async/pvr/waterfall_without/plot
	\begin{subfigure}[b]{0.4\textwidth}
	   \includegraphics[width=1\linewidth]{figs/plot/motiv/async/pvr/waterfall}
	   \caption{A sequence of three GPU commands (top) and the total GPU power (bottom).
	   Commands of the same type have the same color. Hardware: PowerVR SGX544MP}
		\vspace{2mm}
	\end{subfigure}
	\begin{subfigure}[b]{0.4\textwidth}
	   \includegraphics[width=1\linewidth]{figs/plot/motiv/dvfs/power}
	   \caption{Comparison of CPU power of the same app when it runs after a CPU idle period and when it runs after a busy period. 
%	   CPU same as (a)
	   }
	\end{subfigure}

\caption{\textbf{Examples of power entanglement}}

\vspace{-10pt}		% use as needed

\label{fig:motiv}
\end{figure}

==> fig-storage.tex <==
% !TeX root = main.tex

\begin{figure}[t!]
	\centering				
	\begin{minipage}[b]{0.25\textwidth}
		\includegraphics[width=1\textwidth]{figs/plot/fs/fs.pdf}
		\subcaption{}
		%		\label{fig:tiger}
	\end{minipage}
	~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
	%(or a blank line to force the subfigure onto a new line)
	\begin{minipage}[b]{0.2\textwidth}
		\includegraphics[width=1\textwidth]{figs/plot/storage-cost/eval-storage.pdf}
		\subcaption{}
	\end{minipage}
\end{figure}

==> fig-workflow.tex <==
% !TeX root = main.tex

\begin{figure}[t!]
\centering
\includegraphics[width=0.45\textwidth{}]{./figs/workflow} 
%\missingfigure[figwidth=6cm]{Workflow}
%\vspace{-10pt}		% use as needed
\caption{The overall workflow of \sys{}. }
\label{tab:benchmarks}
%\vspace{-20pt}		% use as needed
\end{figure}


==> figs/pdfcrop <==
#!/usr/bin/env perl
use strict;
$^W=1; # turn warning on
#
# pdfcrop.pl
#
# Copyright (C) 2002, 2004, 2005, 2008-2012 Heiko Oberdiek.
#
# This program may be distributed and/or modified under the
# conditions of the LaTeX Project Public License, either version 1.2
# of this license or (at your option) any later version.
# The latest version of this license is in
#   http://www.latex-project.org/lppl.txt
# and version 1.2 or later is part of all distributions of LaTeX
# version 1999/12/01 or later.
#
# See file "README" for a list of files that belong to this project.
#
# This file "pdfcrop.pl" may be renamed to "pdfcrop"
# for installation purposes.
#
my $prj         = 'pdfcrop';
my $file        = "$prj.pl";
my $program     = uc($&) if $file =~ /^\w+/;
my $version     = "1.38";
my $date        = "2012/11/02";
my $author      = "Heiko Oberdiek";
my $copyright   = "Copyright (c) 2002-2012 by $author.";
#
# Reqirements: Perl5, Ghostscript
# History:
#   2002/10/30 v1.0:  First release.
#   2002/10/30 v1.1:  Option --hires added.
#   2002/11/04 v1.2:  "nul" instead of "/dev/null" for windows.
#   2002/11/23 v1.3:  Use of File::Spec module's "devnull" call.
#   2002/11/29 v1.4:  Option --papersize added.
#   2004/06/24 v1.5:  Clear map file entries so that pdfTeX
#                     does not touch the fonts.
#   2004/06/26 v1.6:  Use mgs.exe instead of gswin32c.exe for MIKTEX.
#   2005/03/11 v1.7:  Support of spaces in file names
#                     (open("-|") is used for ghostscript call).
#   2008/01/09 v1.8:  Fix for moving the temporary file to the output
#                     file across file system boundaries.
#   2008/04/05 v1.9:  Options --resolution and --bbox added.
#   2008/07/16 v1.10: Support for XeTeX added with new options
#                     --pdftex, --xetex, and --xetexcmd.
#   2008/07/22 v1.11: Workaround for open("-|").
#   2008/07/23 v1.12: Workarounds for the workaround (error detection, ...).
#   2008/07/24 v1.13: open("-|")/workaround removed.
#                     Input files with unsafe file names are linked/copied
#                     to temporary file with safe file name.
#   2008/09/12 v1.14: Error detection for invalid Bounding Boxes.
#   2009/07/14 v1.15: Fix for negative coordinates in Bounding Boxes
#                     (David Menestrina).
#   2009/07/16 v1.16: Security fixes:
#                     * -dSAFER added for Ghostscript,
#                     * -no-shell-escape added for pdfTeX/XeTeX.
#   2009/07/17 v1.17: Security fixes:
#                     * Backticks and whitespace are forbidden
#                       for options --(gs|pdftex|xetex)cmd.
#                     * Validation of options --papersize and --resolution.
#   2009/07/18 v1.18: * Restricted mode added.
#                     * Option --version added.
#   2009/09/24 v1.19: * Ghostscript detection rewritten.
#                     * Cygwin: `gs' is preferred to `gswin32c'.
#   2009/10/06 v1.20: * File name sanitizing in .tex file.
#   2009/12/21 v1.21: * Option --ini added for IniTeX mode.
#                     * Option --luatex and --luatexcmd added for LuaTeX.
#   2009/12/29 v1.22: * Syntax description for option --bbox fixed
#                       (Lukas Prochazka).
#   2010/01/09 v1.23: * Options --bbox-odd and -bbox-even added.
#   2010/08/16 v1.24: * Workaround added for buggy ghostscript ports
#                       that print the BoundingBox data twice.
#   2010/08/26 v1.25: * Fix for the case that the PDF file contains
#                       an entry /CropBox different to /MediaBox.
#                     * \pageinclude implemented for XeTeX.
#                     * XeTeX: --clip does not die, but this option
#                       is ignored, because XeTeX always clip.
# 2010/08/26 v1.26: * XeTeX's \XeTeXpdffile expects keyword
#                     `media', not `mediabox'.
#                   * New option --pdfversion.
#                     Default is `auto' that means the PDF version
#                     is inherited from the input file. Before
#                     pdfcrop has used the TeX engine's default.
#                   * Option --luatex fixed (extra empty page at end).
# 2010/09/03 v1.27: * Workaround of v1.24 fixed.
# 2010/09/06 v1.28: * The Windows registry is searched if Ghostscript
#                     is not found via PATH.
#                   * Windows only: support of spaces in command
#                     names in unrestricted mode.
# 2010/09/06 v1.29: * Find the latest Ghostscript version in registry.
# 2010/09/15 v1.30: * Warning of pdfTeX because of \pdfobjcompresslevel
#                     avoided when reducing \pdfminorversion.
#                   * Fix for TeX syntax characters in input file names.
# 2010/09/17 v1.31: * Passing the input file name via hex string to TeX.
#                   * Again input file names restricted for Ghostscript
#                     command line, switch then to symbol link/copy
#                     method.
# 2011/08/10 v1.32: * Detection for gswin64c.exe added.
# 2012/02/01 v1.33: * Input file can be `-' (standard input).
# 2012/04/18 v1.34: * Format of --version changed
#                     from naked version number to a line with
#                     program name, date and version.
# 2012/10/15 v1.35: * Additional debug infos added for Perl version.
# 2012/10/16 v1.36: * More error codes added.
# 2012/10/16 v1.37: * Extended error messages if available.
#                   * Fix for broken v1.36.
# 2012/11/02 v1.38: * Fix for unsufficient cleanup, if function `cleanup' is
#                     prematurely called in `eval' for `symlink' checking.

### program identification
my $title = "$program $version, $date - $copyright\n";

### error strings
my $Error = "!!! Error:"; # error prefix

### make ENV safer
delete @ENV{qw(IFS CDPATH ENV BASH_ENV)};

# Windows detection (no SIGHUP)
my $Win = 0;
$Win = 1 if $^O =~ /mswin32/i;
$Win = 1 if $^O =~ /cygwin/i;
use Config;
my $archname = $Config{'archname'};
$archname = 'unknown' unless defined $Config{'archname'};

### extended error messages
sub exterr () {
    chomp(my $msg_errno = $!);
    chomp(my $msg_extended_os_error = $^E);
    if ($msg_errno eq $msg_extended_os_error) {
        $msg_errno;
    }
    else {
        "$msg_errno/$msg_extended_os_error";
    }
}

### string constants for Ghostscript run
# get Ghostscript command name
$::opt_gscmd = '';
sub find_ghostscript () {
    return if $::opt_gscmd;
    if ($::opt_debug) {
        print "* Perl executable: $^X\n";
        if ($] < 5.006) {
            print "* Perl version: $]\n";
        }
        else {
            printf "* Perl version: v%vd\n", $^V;
        }
        if (defined &ActivePerl::BUILD) {
            printf "* Perl product: ActivePerl, build %s\n", ActivePerl::BUILD();
        }
        use Config;
        printf "* Pointer size: $Config{'ptrsize'}\n";
        printf "* Pipe support: %s\n",
                (defined($Config{'d_pipe'}) ? 'yes' : 'no');
        printf "* Fork support: %s\n",
                (defined($Config{'d_fork'}) ? 'yes' : 'no');
    }
    my $system = 'unix';
    $system = "dos" if $^O =~ /dos/i;
    $system = "os2" if $^O =~ /os2/i;
    $system = "win" if $^O =~ /mswin32/i;
    $system = "cygwin" if $^O =~ /cygwin/i;
    $system = "miktex" if defined($ENV{"TEXSYSTEM"}) and
                          $ENV{"TEXSYSTEM"} =~ /miktex/i;
    print "* OS name: $^O\n" if $::opt_debug;
    print "* Arch name: $archname\n" if $::opt_debug;
    print "* System: $system\n" if $::opt_debug;
    my %candidates = (
        'unix' => [qw|gs gsc|],
        'dos' => [qw|gs386 gs|],
        'os2' => [qw|gsos2 gs|],
        'win' => [qw|gswin32c gs|],
        'cygwin' => [qw|gs gswin32c|],
        'miktex' => [qw|mgs gswin32c gs|]
    );
    if ($system eq 'win' or $system eq 'cygwin' or $system eq 'miktex') {
        if ($archname =~ /mswin32-x64/i) {
            my @a = ();
            foreach my $name (@{$candidates{$system}}) {
                push @a, 'gswin64c' if $name eq 'gswin32c';
                push @a, $name;
            }
            $candidates{$system} = \@a;
        }
    }
    my %ext = (
        'unix' => '',
        'dos' => '.exe',
        'os2' => '.exe',
        'win' => '.exe',
        'cygwin' => '.exe',
        'miktex' => '.exe'
    );
    my $candidates_ref = $candidates{$system};
    my $ext = $Config{'_exe'};
    $ext = $ext{$system} unless defined $ext;
    use File::Spec;
    my @path = File::Spec->path();
    my $found = 0;
    foreach my $candidate (@$candidates_ref) {
        foreach my $dir (@path) {
            my $file = File::Spec->catfile($dir, "$candidate$ext");
            if (-x $file) {
                $::opt_gscmd = $candidate;
                $found = 1;
                print "* Found ($candidate): $file\n" if $::opt_debug;
                last;
            }
            print "* Not found ($candidate): $file\n" if $::opt_debug;
        }
        last if $found;
    }
    if (not $found and $Win) {
        $found = SearchRegistry();
    }
    if ($found) {
        print "* Autodetected ghostscript command: $::opt_gscmd\n" if $::opt_debug;
    }
    else {
        $::opt_gscmd = $$candidates_ref[0];
        print "* Default ghostscript command: $::opt_gscmd\n" if $::opt_debug;
    }
}

sub SearchRegistry () {
    my $found = 0;
    eval 'use Win32::TieRegistry qw|KEY_READ REG_SZ|;';
    if ($@) {
        if ($::opt_debug) {
            print "* Registry lookup for Ghostscript failed:\n";
            my $msg = $@;
            $msg =~ s/\s+$//;
            foreach (split /\r?\n/, $msg) {
                print "  $_\n";
            }
        }
        return $found;
    }
    my $open_params = {Access => KEY_READ(), Delimiter => '/'};
    my $key_name_software = 'HKEY_LOCAL_MACHINE/SOFTWARE/';
    my $current_key = $key_name_software;
    my $software = new Win32::TieRegistry $current_key, $open_params;
    if (not $software) {
        print "* Cannot find or access registry key `$current_key'!\n"
                if $::opt_verbose;
        return $found;
    }
    print "* Search registry at `$current_key'.\n" if $::opt_debug;
    my %list;
    foreach my $key_name_gs (grep /Ghostscript/i, $software->SubKeyNames()) {
        $current_key = "$key_name_software$key_name_gs/";
        print "* Registry entry found: $current_key\n" if $::opt_debug;
        my $key_gs = $software->Open($key_name_gs, $open_params);
        if (not $key_gs) {
            print "* Cannot open registry key `$current_key'!\n" if $::opt_debug;
            next;
        }
        foreach my $key_name_version ($key_gs->SubKeyNames()) {
            $current_key = "$key_name_software$key_name_gs/$key_name_version/";
            print "* Registry entry found: $current_key\n" if $::opt_debug;
            if (not $key_name_version =~ /^(\d+)\.(\d+)$/) {
                print "  The sub key is not a version number!\n" if $::opt_debug;
                next;
            }
            my $version_main = $1;
            my $version_sub = $2;
            $current_key = "$key_name_software$key_name_gs/$key_name_version/";
            my $key_version = $key_gs->Open($key_name_version, $open_params);
            if (not $key_version) {
                print "* Cannot open registry key `$current_key'!\n" if $::opt_debug;
                next;
            }
            $key_version->FixSzNulls(1);
            my ($value, $type) = $key_version->GetValue('GS_DLL');
            if ($value and $type == REG_SZ()) {
                print "  GS_DLL = $value\n" if $::opt_debug;
                $value =~ s|([\\/])([^\\/]+\.dll)$|$1gswin32c.exe|i;
                my $value64 = $value;
                $value64 =~ s/gswin32c\.exe$/gswin64c.exe/;
                if ($archname =~ /mswin32-x64/i and -f $value64) {
                    $value = $value64;
                }
                if (-f $value) {
                    print "  EXE found: $value\n" if $::opt_debug;
                }
                else {
                    print "  EXE not found!\n" if $::opt_debug;
                    next;
                }
                my $sortkey = sprintf '%02d.%03d %s',
                        $version_main, $version_sub, $key_name_gs;
                $list{$sortkey} = $value;
            }
            else {
                print "  Missing key `GS_DLL' with type `REG_SZ'!\n" if $::opt_debug;
            }
        }
    }
    foreach my $entry (reverse sort keys %list) {
        $::opt_gscmd = $list{$entry};
        print "* Found (via registry): $::opt_gscmd\n" if $::opt_debug;
        $found = 1;
        last;
    }
    return $found;
}

# restricted mode
my $restricted = 0;
if ($0 =~ /rpdfcrop/ or $0 =~ /restricted/) {
    $restricted = 1;
}

# "null" device
use File::Spec::Functions qw(devnull);
my $null = devnull();

### variables
my $inputfile   = "";
my $outputfile  = "";
my $tmp = "tmp-\L$program\E-$$";

### paper sizes

my @papersizes = qw[
  11x17 ledger legal letter lettersmall
  archE archD archC archB archA
  a0 a1 a2 a3 a4 a4small a5 a6 a7 a8 a9 a10
  isob0 isob1 isob2 isob3 isob4 isob5 isob6
  c0 c1 c2 c3 c4 c5 c6
  jisb0 jisb1 jisb2 jisb3 jisb4 jisb5 jisb6
  b0 b1 b2 b3 b4 b5
  flsa flse halfletter
];
my %papersizes;
foreach (@papersizes) {
    $papersizes{$_} = 1;
}

### option variables
my @bool = ("false", "true");
$::opt_version    = 0;
$::opt_help       = 0;
$::opt_debug      = 0;
$::opt_verbose    = 0;
$::opt_pdftexcmd  = "pdftex";
$::opt_xetexcmd   = "xetex";
$::opt_luatexcmd  = "luatex";
$::opt_tex        = "pdftex";
$::opt_margins    = "0 0 0 0";
$::opt_clip       = 0;
$::opt_hires      = 0;
$::opt_papersize  = "";
$::opt_resolution = "";
$::opt_bbox       = "";
$::opt_bbox_odd   = "";
$::opt_bbox_even  = "";
$::opt_initex     = 0;
$::opt_pdfversion = "auto";

sub usage ($) {
    my $ret = shift;
    find_ghostscript();
    my $usage = <<"END_OF_USAGE";
${title}Syntax:   \L$program\E [options] <input[.pdf]> [output file]
Function: Margins are calculated and removed for each page in the file.
Options:                                                       (defaults:)
  --help              print usage
  --version           print version number
  --(no)verbose       verbose printing                         ($bool[$::opt_verbose])
  --(no)debug         debug informations                       ($bool[$::opt_debug])
  --gscmd <name>      call of ghostscript                      ($::opt_gscmd)
  --pdftex | --xetex | --luatex
                      use pdfTeX | use XeTeX | use LuaTeX      ($::opt_tex)
  --pdftexcmd <name>  call of pdfTeX                           ($::opt_pdftexcmd)
  --xetexcmd <name>   call of XeTeX                            ($::opt_xetexcmd)
  --luatexcmd <name>  call of LuaTeX                           ($::opt_luatexcmd)
  --margins "<left> <top> <right> <bottom>"                    ($::opt_margins)
                      add extra margins, unit is bp. If only one number is
                      given, then it is used for all margins, in the case
                      of two numbers they are also used for right and bottom.
  --(no)clip          clipping support, if margins are set     ($bool[$::opt_clip])
                      (not available for --xetex)
  --(no)hires         using `%%HiResBoundingBox'               ($bool[$::opt_hires])
                      instead of `%%BoundingBox'
  --(no)ini           use iniTeX variant of the TeX compiler   ($bool[$::opt_initex])
Expert options:
  --restricted        turn on restricted mode                  ($bool[$restricted])
  --papersize <foo>   parameter for gs's -sPAPERSIZE=<foo>,
                      use only with older gs versions <7.32    ($::opt_papersize)
  --resolution <xres>x<yres>                                   ($::opt_resolution)
  --resolution <res>  pass argument to ghostscript's option -r
                      Example: --resolution 72
  --bbox "<left> <bottom> <right> <top>"                       ($::opt_bbox)
                      override bounding box found by ghostscript
                      with origin at the lower left corner
  --bbox-odd          Same as --bbox, but for odd pages only   ($::opt_bbox_odd)
  --bbox-even         Same as --bbox, but for even pages only  ($::opt_bbox_even)
  --pdfversion <1.x> | auto | none
                      Set the PDF version to 1.x, 1 < x < 8.
                      If `auto' is given as value, then the
                      PDF version is taken from the header
                      of the input PDF file.
                      An empty value or `none' uses the
                      default of the TeX engine.               ($::opt_pdfversion)

Input file: If the name is `-', then the standard input is used and
  the output file name must be explicitly given.
Examples:
  \L$program\E --margins 10 input.pdf output.pdf
  \L$program\E --margins '5 10 5 20' --clip input.pdf output.pdf
In case of errors:
  Try option --verbose first to get more information.
In case of bugs:
  Please, use option --debug for bug reports.
END_OF_USAGE
    if ($ret) {
        die $usage;
    }
    else {
        print $usage;
        exit(0);
    }
}

### process options
my @OrgArgv = @ARGV;
use Getopt::Long;
GetOptions(
  "help!",
  "version!",
  "debug!",
  "verbose!",
  "gscmd=s",
  "pdftexcmd=s",
  "xetexcmd=s",
  "luatexcmd=s",
  "pdftex" => sub { $::opt_tex = 'pdftex'; },
  "xetex"  => sub { $::opt_tex = 'xetex'; },
  "luatex" => sub { $::opt_tex = 'luatex'; },
  "initex!",
  "margins=s",
  "clip!",
  "hires!",
  "papersize=s",
  "resolution=s",
  "bbox=s",
  "bbox-odd=s" => \$::opt_bbox_odd,
  "bbox-even=s" => \$::opt_bbox_even,
  "restricted" => sub { $restricted = 1; },
  "pdfversion=s" => \$::opt_pdfversion,
) or usage(1);
!$::opt_help or usage(0);

if ($::opt_version) {
    print "$prj $date v$version\n";
    exit(0);
}

$::opt_verbose = 1 if $::opt_debug;

@ARGV >= 1 or usage(1);

print $title;

print "* Restricted mode: ", ($restricted ? "enabled" : "disabled"), "\n"
        if $::opt_debug;

$::opt_pdfversion =~ /^(|none|auto|1\.([2-7]))$/
        or die "!!! Error: Invalid value `$::opt_pdfversion' for option `--pdfversion'!\n";
print "* Option `pdfversion': $::opt_pdfversion\n" if $::opt_debug;
$::opt_pdfversion = $2 if $2;
$::opt_pdfversion = '' if $::opt_pdfversion eq 'none';

find_ghostscript();

if ($::opt_bbox) {
    $::opt_bbox =~ s/^\s+//;
    $::opt_bbox =~ s/\s+$//;
    $::opt_bbox =~ s/\s+/ /;
    if ($::opt_bbox =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box: $::opt_bbox\n" if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox \"$::opt_bbox\")!\n";
    }
}
if ($::opt_bbox_odd) {
    $::opt_bbox_odd =~ s/^\s+//;
    $::opt_bbox_odd =~ s/\s+$//;
    $::opt_bbox_odd =~ s/\s+/ /;
    if ($::opt_bbox_odd =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box for odd pages: $::opt_bbox_odd\n"
                if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox-odd \"$::opt_bbox_odd\")!\n";
    }
}
if ($::opt_bbox_even) {
    $::opt_bbox_even =~ s/^\s+//;
    $::opt_bbox_even =~ s/\s+$//;
    $::opt_bbox_even =~ s/\s+/ /;
    if ($::opt_bbox_even =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box for even pages: $::opt_bbox_even\n"
                if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox-even \"$::opt_bbox_even\")!\n";
    }
}

@ARGV <= 2 or die "$Error Too many files!\n";

### input file
$inputfile = shift @ARGV;

if ($inputfile eq '-') {
    @ARGV == 1 or die "$Error Missing output file name!\n";
    print "* Input file: <stdin>\n" if $::opt_debug;
}
else {
    if (! -f $inputfile) {
        if (-f "$inputfile.pdf") {
            $inputfile .= ".pdf";
        }
        else {
            die "$Error Input file `$inputfile' not found!\n";
        }
    }
    print "* Input file: $inputfile\n" if $::opt_debug;
}

### output file
if (@ARGV) {
    $outputfile = shift @ARGV;
}
else {
    $outputfile = $inputfile;
    $outputfile =~ s/\.pdf$//i;
    $outputfile .= "-crop.pdf";
}

print "* Output file: $outputfile\n" if $::opt_debug;

### margins
my ($llx, $lly, $urx, $ury) = (0, 0, 0, 0);
if ($::opt_margins =~
        /^\s*([\-\.\d]+)\s+([\-\.\d]+)\s+([\-\.\d]+)\s+([\-\.\d]+)\s*$/) {
    ($llx, $lly, $urx, $ury) = ($1, $2, $3, $4);
}
else {
    if ($::opt_margins =~ /^\s*([\-\.\d]+)\s+([\-\.\d]+)\s*$/) {
        ($llx, $lly, $urx, $ury) = ($1, $2, $1, $2);
    }
    else {
        if ($::opt_margins =~ /^\s*([\-\.\d]+)\s*$/) {
            ($llx, $lly, $urx, $ury) = ($1, $1, $1, $1);
        }
        else {
            die "$Error Parse error (option --margins)!\n";
        }
    }
}
print "* Margins: $llx $lly $urx $ury\n" if $::opt_debug;

### papersize validation (security)
if ($::opt_papersize ne '') {
    $::opt_papersize =~ /^[0-9A-Za-z]+$/
            or die "$Error Invalid papersize ($::opt_papersize)!\n";
    $papersizes{$::opt_papersize}
            or die "$Error Unknown papersize ($::opt_papersize),"
                   . " see ghostscript's documentation for option `-r'!\n";
}

### resolution validation (security)
if ($::opt_resolution ne '') {
    $::opt_resolution =~ /^\d+(x\d+)?$/
            or die "$Error Invalid resolution ($::opt_resolution),"
                   . " see ghostscript's documentation!\n";
}

### command name validation (security)
my %cmd = (
    'gscmd' => \$::opt_gscmd,
    'pdftexcmd' => \$::opt_pdftexcmd,
    'luatexcmd' => \$::opt_luatexcmd,
    'xetexcmd' => \$::opt_xetexcmd
);
foreach my $cmd (keys %cmd) {
    my $cmd_ref = $cmd{$cmd};
    $$cmd_ref =~ s/^\s+//;
    $$cmd_ref =~ s/\s+$//;
    my $val = $$cmd_ref;
    next unless $val;
    next unless $val;
    if ($val =~ /`/) {
        die "$Error Forbidden backtick for option `--$cmd' ($val)!\n";
    }
    if ($val =~ /\s/) {
        my $err = 0;
        if ($restricted or not $Win) {
            $err = 1;
        }
        else {
            $err = 1 if $val =~ /\.exe.*\s/i;
            $err = 1 if $val =~ /\s[-\/@+]/;
        }
        die "$Error Forbidden whitespace for option `--$cmd' ($val)!\n" if $err;
    }
}
if ($restricted) {
    if ($::opt_pdftexcmd and $::opt_pdftexcmd ne 'pdftex') {
        die "$Error pdfTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_xetexcmd and $::opt_xetexcmd ne 'xetex') {
        die "$Error XeTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_luatexcmd and $::opt_luatexcmd ne 'luatex') {
        die "$Error LuaTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_gscmd) {
        $::opt_gscmd =~ /^(gs|mgs|gswin32c|gs386|gsos2)$/
        or $::opt_gscmd =~ /^gs[\-_]?(\d|\d[\.-_]?\d\d)c?$/
        or die "$Error: Invalid Ghostscript program name in restricted mode!\n";
    }
}
if ($Win and $::opt_gscmd =~ /\s/) {
    $::opt_gscmd = "\"$::opt_gscmd\"";
}

### cleanup system
my @unlink_files = ();
my $exit_code = 1;
sub clean {
    print "* Cleanup\n" if $::opt_debug;
    if ($::opt_debug) {
        print "* Temporary files: @unlink_files\n";
    }
    else {
        for (; @unlink_files>0; ) {
            unlink shift @unlink_files;
        }
    }
}
sub cleanup {
    clean();
    exit($exit_code);
}
$SIG{'INT'} = \&cleanup;
$SIG{'__DIE__'} = \&clean;

### Calculation of BoundingBoxes

# use safe file name for use within cmd line of gs (unknown shell: space, ...)
# and XeTeX (hash, curly braces, ...)
my $inputfilesafe = $inputfile;
if ($inputfile eq '-') {
    $inputfilesafe = "$tmp-stdin.pdf";
    print "* Temporary input file: $inputfilesafe\n" if $::opt_debug;
    push @unlink_files, $inputfilesafe;
    open(OUT, '>', $inputfilesafe)
            or die sprintf "$Error Cannot write `%s' (%s)!\n",
                           $inputfilesafe, exterr;
    binmode(OUT);
    my $size = 0;
    my $len = 0;
    my $buf = '';
    my $buf_size = 65536;
    do {
        $len = read STDIN, $buf, $buf_size;
        if (not defined $len) {
            my $msg = exterr;
            die "$Error Reading standard input ($msg)!\n";
        }
        print OUT $buf
                or die sprintf "$Error Writing `%s` (%s)!\n",
                               $inputfilesafe, exterr;
        $size += $len;
    }
    while ($len);
    close(OUT);
    print "* File size (STDIN): $size\n" if $::opt_debug;
}
elsif (not $inputfile =~ /^[\w\d\.\-\:\/@]+$/) { # /[\s\$~'"#{}%]/
    $inputfilesafe = "$tmp-img.pdf";
    push @unlink_files, $inputfilesafe;
    my $symlink_exists = eval {
        local $SIG{'__DIE__'};
        symlink("", "");
        1;
    };
    print "* Input file name `$inputfile' contains special characters.\n"
          . "* " . ($symlink_exists ? "Link" : "Copy")
          . " input file to temporary file `$inputfilesafe'.\n"
            if $::opt_verbose;
    if ($symlink_exists) {
        symlink($inputfile, $inputfilesafe)
            or die sprintf "$Error Link from `%s' to `%s' failed (%s)!\n",
                           $inputfile, $inputfilesafe, exterr;
    }
    else {
        use File::Copy;
        copy($inputfile, $inputfilesafe)
                or die sprintf "$Error Copy from `%s' to `%s' failed (%s)\n",
                               $inputfile, $inputfilesafe, exterr;
    }
}

if ($::opt_pdfversion eq 'auto') {
    open(IN, '<', $inputfilesafe)
            or die sprintf "!!! Error: Cannot open `%s' (%s)!\n",
                           $inputfilesafe, exterr;
    my $buf;
    read(IN, $buf, 1024)
            or die sprintf "!!! Error: Cannot read the header of `%s' failed (%s)!\n",
                           $inputfilesafe, exterr;
    close(IN);
    if ($buf =~ /%PDF-1.([0-7])\s/) {
        $::opt_pdfversion = $1;
        print "* PDF header: %PDF-1.$::opt_pdfversion\n" if $::opt_verbose;
        $::opt_pdfversion = 2 if $::opt_pdfversion < 2;
    }
    else {
        die "!!! Error: Cannot find PDF header of `$inputfilesafe'!\n";
    }
}
print '* Using PDF minor version: ',
      ($::opt_pdfversion ? $::opt_pdfversion : "engine's default"),
      "\n" if $::opt_debug;

my @gsargs = (
    "-sDEVICE=bbox",
    "-dBATCH",
    "-dNOPAUSE"
);
push @gsargs, "-sPAPERSIZE=$::opt_papersize" if $::opt_papersize;
push @gsargs, "-r$::opt_resolution" if $::opt_resolution;
push @gsargs,
    "-c",
    "save",
    "pop",
    "-f",
    $inputfilesafe
;

my $tmpfile = "$tmp.tex";
push @unlink_files, $tmpfile;
open(TMP, ">$tmpfile")
    or die sprintf "$Error Cannot write tmp file `%s' (%s)!\n",
                   $tmpfile, exterr;
print TMP <<'END_TMP';
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
END_TMP
my $pdffilehex = unpack 'H*', $inputfilesafe;
$pdffilehex = "\U$pdffilehex\E";
print TMP "\\def\\pdffilehex{$pdffilehex}\n";
print TMP <<'END_TMP';
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
END_TMP
if ($::opt_tex eq 'luatex') {
    print TMP <<'END_TMP';
\begingroup\expandafter\expandafter\expandafter\endgroup
\expandafter\ifx\csname directlua\endcsname\relax
  \errmessage{LuaTeX not found!}%
\else
  \begingroup
    \newlinechar=10 %
    \endlinechar=\newlinechar %
    \ifnum0%
        \directlua{%
          if tex.enableprimitives then
            tex.enableprimitives('TEST', {
              'luatexversion',
              'pdfoutput',
              'pdfcompresslevel',
              'pdfhorigin',
              'pdfvorigin',
              'pdfpagewidth',
              'pdfpageheight',
              'pdfmapfile',
              'pdfximage',
              'pdflastximage',
              'pdfrefximage',
              'pdfminorversion',
              'pdfobjcompresslevel',
            })
            tex.print('1')
          end
        }%
        \ifx\TESTluatexversion\UnDeFiNeD\else 1\fi %
        =11 %
      \global\let\luatexversion\luatexversion %
      \global\let\pdfoutput\TESTpdfoutput %
      \global\let\pdfcompresslevel\TESTpdfcompresslevel %
      \global\let\pdfhorigin\TESTpdfhorigin %
      \global\let\pdfvorigin\TESTpdfvorigin %
      \global\let\pdfpagewidth\TESTpdfpagewidth %
      \global\let\pdfpageheight\TESTpdfpageheight %
      \global\let\pdfmapfile\TESTpdfmapfile %
      \global\let\pdfximage\TESTpdfximage %
      \global\let\pdflastximage\TESTpdflastximage %
      \global\let\pdfrefximage\TESTpdfrefximage %
      \global\let\pdfminorversion\TESTpdfminorversion %
      \global\let\pdfobjcompresslevel\TESTpdfobjcompresslevel %
    \else %
      \errmessage{%
        Missing \string\luatexversion %
      }%
    \fi %
  \endgroup %
\fi
END_TMP
}
if ($::opt_tex eq 'pdftex' or $::opt_tex eq 'luatex') {
    print TMP <<'END_TMP_HEAD';
\pdfoutput=1 %
\pdfcompresslevel=9 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1<5 %
      \pdfobjcompresslevel=0 %
    \else
      \pdfobjcompresslevel=2 %
    \fi
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#1\relax
    }%
  }{%
    \pdfminorversion=#1\relax
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
END_TMP_HEAD
    print TMP "\\setpdfversion{$::opt_pdfversion}\n" if $::opt_pdfversion;
}
else { # XeTeX
    print TMP <<'END_TMP_HEAD';
\expandafter\ifx\csname XeTeXpdffile\endcsname\relax
  \errmessage{XeTeX not found or too old!}%
\fi
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \XeTeXpdffile "\pdffile" page #1 media\relax
  }%
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \shipout\hbox{%
    \kern-1in%
    \kern-#2bp%
    \vbox{%
      \kern-1in%
      \kern#3bp%
      \ht0=\pdfpageheight
      \box0 %
    }%
  }%
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \page {#1} [#2 #3 #4 #5]%
}
\def\pageinclude#1{%
  \setbox0=\hbox{%
    \XeTeXpdffile "\pdffile" page #1 media\relax
  }%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \kern-1in%
    \vbox{%
      \kern-1in%
      \ht0=\pdfpageheight
      \box0 %
    }%
  }%
}
END_TMP_HEAD
}

print "* Running ghostscript for BoundingBox calculation ...\n"
    if $::opt_verbose;
print "* Ghostscript call: $::opt_gscmd @gsargs\n" if $::opt_debug;

my @bbox;
my @bbox_all;
my @bbox_odd;
my @bbox_even;
if ($::opt_bbox) {
     $::opt_bbox =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_all = ($1, $2, $3, $4);
}
if ($::opt_bbox_odd) {
     $::opt_bbox_odd =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_odd = ($1, $2, $3, $4);
}
if ($::opt_bbox_even) {
     $::opt_bbox_even =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_even = ($1, $2, $3, $4);
}

sub getbbox ($$$$$) {
    my $page = shift;
    my $a = shift;
    my $b = shift;
    my $c = shift;
    my $d = shift;
    if ($page % 2 == 1) {
        if ($::opt_bbox_odd) {
            return @bbox_odd;
        }
    }
    else {
        if ($::opt_bbox_even) {
            return @bbox_even;
        }
    }
    if ($::opt_bbox) {
        return @bbox_all;
    }
    return ($a, $b, $c, $d);
}
my $page = 0;
my $gs_pipe = "$::opt_gscmd -dSAFER @gsargs 2>&1";
$gs_pipe .= " 1>$null" unless $::opt_verbose;
$gs_pipe .= " |";

open(GS, $gs_pipe)
        or die sprintf "$Error Cannot call ghostscript `%s' (%s)!\n",
                       $::opt_gscmd, exterr;
my $bb = ($::opt_hires) ? "%%HiResBoundingBox" : "%%BoundingBox";
my $previous_line = 'Previous line';
# Ghostscript workaround for buggy ports that prints
# the bounding box data twice on STDERR.
while (<GS>) {
    print $_ if $::opt_verbose;
    if (/^$bb:\s*(-?[\.\d]+) (-?[\.\d]+) (-?[\.\d]+) (-?[\.\d]+)/o) {
    }
    else {
        $previous_line = $_;
        next;
    }
    next if $previous_line eq $_;
    $previous_line = $_;
    $page++;
    @bbox = getbbox($page, $1, $2, $3, $4);

    my $empty = 0;
    $empty = 1 if $bbox[0] >= $bbox[2];
    $empty = 1 if $bbox[1] >= $bbox[3];
    if ($empty) {
        print <<"END_WARNING";

!!! Warning: Empty Bounding Box is returned by Ghostscript!
!!!   Page $page: @bbox
!!! Either there is a problem with the page or with Ghostscript.
!!! Recovery is tried by embedding the page in its original size.

END_WARNING
        print TMP "\\pageinclude{$page}\n";
        next;
    }

    print "* Page $page: @bbox\n" if $::opt_verbose;

    my @bb = ($bbox[0] - $llx, $bbox[1] - $ury,
             $bbox[2] + $urx, $bbox[3] + $lly);

    $empty = 0;
    $empty = 1 if $bb[0] >= $bb[2];
    $empty = 1 if $bb[1] >= $bb[3];
    if ($empty) {
        print <<"END_WARNING";

!!! Warning: The final Bounding Box is empty!
!!!   Page: $page: @bb
!!! Probably caused by too large negative margin values.
!!! Recovery by ignoring margin values.

END_WARNING
        print TMP "\\page $page [@bbox]\n";
        # clipping shouldn't make a difference
        next;
    }
    if ($::opt_clip) {
        print TMP "\\pageclip $page [@bbox][$llx $lly $urx $ury]\n";
    }
    else {
        print TMP "\\page $page [@bb]\n";
    }
}
close(GS);

if ($? == -1) {
    die sprintf "$Error Ghostscript failed to execute (%s)!\n",
                exterr;
}
elsif ($? & 127) {
    die sprintf  "$Error Ghostscript died with signal %d!\n",
                 ($? & 127);
}
elsif ($? != 0) {
    die sprintf "$Error Ghostscript exited with error code %d!\n",
                $? >> 8;
}

print TMP "\\csname \@\@end\\endcsname\n\\end\n";
close(TMP);

if ($page == 0) {
    die "$Error Ghostscript does not report bounding boxes!\n";
}

### Run pdfTeX/XeTeX

push @unlink_files, "$tmp.log";
my $cmd;
my $texname;
if ($::opt_tex eq 'pdftex') {
    $cmd = $::opt_pdftexcmd;
    $texname = 'pdfTeX';
}
elsif ($::opt_tex eq 'luatex') {
    $cmd = $::opt_luatexcmd;
    $texname = 'LuaTeX';
}
else {
    $cmd = $::opt_xetexcmd;
    $texname = 'XeTeX';
}
$cmd = "\"$cmd\"" if $Win and $cmd =~ /\s/;
$cmd .= ' -no-shell-escape';
if ($::opt_initex) {
    $cmd .= ' --ini --etex';
}
if ($::opt_verbose) {
    $cmd .= " -interaction=nonstopmode $tmp";
}
else {
    $cmd .= " -interaction=batchmode $tmp";
}
print "* Running $texname ...\n" if $::opt_verbose;
print "* $texname call: $cmd\n" if $::opt_debug;
if ($::opt_verbose) {
    system($cmd);
}
else {
    `$cmd`;
}
if ($? == -1) {
    die sprintf "$Error %s run failed to execute (%s)!\n",
                $texname, exterr;
}
elsif ($? & 127) {
    die sprintf "$Error %s run died with signal %d!\n",
                $texname, ($? & 127);
}
elsif ($? != 0) {
    die sprintf "$Error %s run failed with value %d!\n",
                $texname, ($? >> 8);
}

### Check pdf version of temp file
if ($::opt_pdfversion) {
    open(PDF, '+<', "$tmp.pdf")
            or die sprintf "!!! Error: Cannot open `%s' (%s)!\n",
                           "$tmp.pdf", exterr;
    my $header;
    read PDF, $header, 9
            or die sprintf "!!! Error: Cannot read header of `%s' (%s)!\n",
                           "$tmp.pdf", exterr;
    $header =~ /^%PDF-1\.(\d)\s$/ or die "!!! Error: Cannot find header of `$tmp.pdf'!\n";
    if ($1 ne $::opt_pdfversion) {
        seek PDF, 7, 0
                or die sprintf "!!! Error: Cannot seek in `%s' (%s)!\n",
                               "$tmp.pdf", exterr;
        print PDF $::opt_pdfversion
                or die sprintf "!!! Error: Cannot write in `%s' (%s)!\n",
                               "$tmp.pdf", exterr;
        print "* PDF version correction in output file: 1.$::opt_pdfversion\n"
                if $::opt_debug;
    }
    close(PDF);
}

### Move temp file to output
if (!rename("$tmp.pdf", $outputfile)) {
    use File::Copy;
    move "$tmp.pdf", $outputfile or
            die "$Error Cannot move `$tmp.pdf' to `$outputfile'!\n";
}

print "==> $page page", (($page == 1) ? "" : "s"),
      " written on `$outputfile'.\n";

$exit_code = 0;
cleanup();

__END__


==> list-fc.tex <==
% !TeX root = main.tex

% ref: https://tex.stackexchange.com/questions/144170/lstlistings-reference-to-line-number


\vspace{-1mm}
\lstset{
	language=C++,
%	basicstyle=\ttfamily\footnotesize\small,
	basicstyle=\fontsize{8}{8}\selectfont\ttfamily,
%	xleftmargin=5.0ex,
%	framexleftmargin=5.0ex,
	frame=tb, % top & bottom
	breaklines=true,
	captionpos=b,
%	numbers=left,
	label=list:attest}
	
%% https://stackoverflow.com/questions/13145368/find-the-maximum-value-in-a-list-of-tuples-in-python
	
\begin{lstlisting}[caption={Sample audit records for the pipeline in Figure~\ref{fig:pipeline-stacked}. Format is simplified. ts means processing timestamp.}, escapechar=!]
//q:quality c:crop r:resolution k:frameskip
q = MAX
for c in crop_factors:
  frontier += search_2D_RxF(q, c, accuracy)
c0,r0,f0,R = min(frontier,key=lambda x:x[R.consume])
while accuracy = profile(op,q,c0,r0,f0) > acc_t
  q = lower() // FIXME
return <q0, c0, r0, k0>  
\end{lstlisting}
\vspace{-2mm}
% uint32_t sort(x_addr *dests, uint32_t n_outputs, x_addr src, idx_t keypos, idx_t reclen);


%for <r, f, R> in frontier: 
%  get where R<consume> is minimum

==> list-fs.tex <==
% !TeX root = main.tex

% ref: https://tex.stackexchange.com/questions/144170/lstlistings-reference-to-line-number


\vspace{-1mm}
\lstset{
	language=C++,
%	basicstyle=\ttfamily\footnotesize\small,
	basicstyle=\fontsize{8}{8}\selectfont\ttfamily,
%	xleftmargin=5.0ex,
%	framexleftmargin=5.0ex,
	frame=tb, % top & bottom
	breaklines=true,
	captionpos=b,
%	numbers=left,
	label=list:attest}
	
%% https://stackoverflow.com/questions/13145368/find-the-maximum-value-in-a-list-of-tuples-in-python
	
\begin{lstlisting}[caption={Sample audit records for the pipeline in Figure~\ref{fig:pipeline-stacked}. Format is simplified. ts means processing timestamp.}, escapechar=!]
//f0,e0 and f1,e1
f2=element-wise_max(f0,f1)
e2=search_2D_(...)
return <e2,f2>
\end{lstlisting}
\vspace{-2mm}
% uint32_t sort(x_addr *dests, uint32_t n_outputs, x_addr src, idx_t keypos, idx_t reclen);


%for <r, f, R> in frontier: 
%  get where R<consume> is minimum

==> model.tex <==
% !TeX root = main.tex

%\section{Configuration}
%\section{Modeling and Building \istream{} Hierarchy}
%\section{Building \istream{} Hierarchy}
\section{Storage Optimizer}
\label{sec:config}

\input{fig-istream-store}

\sys{}'s storage policy is flexible (XXX continuous parameters and 1 binary parameter for each \istream{} and each age span). It creates a huge space that is infeasible for manual exploration. 
For instance, XXXX

We build a model that describes the relation between system configurations, storage policies, and query performance. 
Through the model, we formulate optimal storage policies as an optimization problem for maximizing the query performance utility under given resource constraints. 
With the help of a model solver, 
\sys{} produces storage policies that best mitigate resource bottlenecks in operators, storage, and codec. 

\subsection{Model setup}

\paragraph{Model symbols}
Table~\ref{tab:benchmarks} summarizes the model symbols. 
(including hardware specifications, query profiles, and user-defined weights)

\begin{itemize}

\item \textbf{System configurations (model parameters)}. 
Hardware specifications: 
bandwidth of storage tiers and the decoder (all in input FPS \note{can be tricky, as across different istreams there can be different fidelity}). 
\note{Note that we move decoder to query/operator profiles}
\textit{Ingestion:} 
The system continuously ingests video streams sent from $N_{cam}$ camera(s).
Without loss of generality, we assume all cameras produce the same fidelity (format) of videos (same FPS, resolution, always encoded). 
\textit{Analytics profiles} (come from auto profiling): 
The ideal throughput of each operator (with their desired video fidelity); 
the activation probability (likelihood) of each operator; 
Number of ingestion camera streams. 
\textit{User preference} (from user input): 
timespans for ages and the (global) weights. 
performance weights of multiple queries. 
The system ingests video streams from $N_{cam}$ camera(s).
Without loss of generality, we assume all cameras produce the same fidelity (format) of videos (same FPS, resolution, always encoded). 

\item 
\textbf{Storage policies (model variables to be solved)}: 
For each temp span (of a given istream): 
i) whether it should be stored as encoded; 
ii) the data (chunk) distribution over storage tiers. 
Given an istream: 
$D_t(s)$ is a fraction number. It means among the data of the temperature of $t$, what is the fraction of the data stored on storage type $s$. 
Given a temperature $t$ (e.g. cold), the sum of all fractions should be equal 1: 
$ \sum_s D_t(s) = 1$

\item 
\textbf{Query performance (objective to maximize)}:
We next model the performance of a query running standalone. 
\end{itemize}

\note{todo: a figure showing how things fit together}

\note{move somewhere?}
Second, ingestion IO. The store software/hardware entail bandwidth of storage and codec, which them have  strong impacts on ingestion performance. Each ingested video stream consumes storage bandwidth and optionally codec (transcoding?) bandwidth if the ingested format differs from the storage format. (define format? or fidelity). 

%\subsection{Modeling \istream{}s on tired storage}


\note{``single query''} may be misleading. individual query. 
\sys{} is able to execute multiple queries in parallel. But we model the performance of one query running alone (the typical use cases) and plan resources accordingly. \note{Is this correct?}
Besides, we does not model the query behavior when reconfiguration is running in the background.
The reason is because the current model for running single query is the most basic and common use case, and all other system add-ons can be built upon this model.


%\subsection{Modeling Query Performance}

%Given the hardware resources and queries, an optimization problem will be resolved by a non-linear solver.  For a single \istream{}, it can be distributed on any storage tier. 
%The placement of any single video frame can be evaluated in 4 dimensions:

\input{table-variables}


a nonlinear model?
We assume the number of \istream{}s and their fidelities are already determined (statically) based on query profiles as described in XXX. 

\paragraph{Constraint: ingestion throughput}
%\paragraph{Global ingestion throughput constraints:}
\note{undefined variables}
TBD

There are 2 global constraints on ingestion speed: disk write speed and transcoding speed.
Suppose we have $n$ operators.

On a certain storage tier $s$, the \istream{} configuration bitrate should not exceed the disk write speed. 
We only consider hot video data ingestion because newly ingested videos temperature is by default considered as the highest.
\begin{equation}
	\begin{aligned}
	\sum_{i = 1}^{n}D_{in}(i, s) \times(\verb!En!(i, s, hot) ? B_e(i):B_r(i)) \leq W(s)
	\end{aligned}
\end{equation}
Moreover, the transcoding speed (storing encoded frames) and decode speed (storing raw frames) should also catch up with the ingested frame rate. 
So $\forall i \in n, \forall t \in temperature$, 
\begin{equation}
\verb!En!(i, s, t) ? T_{trans}(i) : T_{decode}(i) \geq fps \times N_{cam}
\end{equation}

\paragraph{Constraint: total storage capacity}
Moreover, the total data size should never exceed the storage limit. (these are global constraints). 
 
Data are distributed on different storage tiers , either as encoded or raw frames.
The total data size of the video stored on tier s of temperature t is：

\begin{equation}
\begin{aligned}
S(i, t) = \mathcal{} L_t  \times D_t(i,s) \times (\verb!En!(i, s, t) ? B_e(i): B_r(i))
\end{aligned}
\end{equation}

Across all data temperatures and resolutions, the total size should not exceed the disk capacity of storage tier $s$.
\begin{equation}
	\begin{aligned}
	\mathcal{} \sum_{t=hot}^{cold} \sum_{i=1}^{n} S(i, t) 
	\leq C_{s}
	\end{aligned}
\end{equation}


%\subsubsection{Objective function: query performance}
%\paragraph{Modeling sketch (roadmap)}
\paragraph{Objective function: query performance}
To derive the overall performance utility $T_{all}$, we describe from the bottom up. 
We first formulate effective IO throughput loading an age span (which is distributed over storage tiers).
We then formulate an operator's throughput in retrieving \& consuming a temp span. 
We then formulate the \st{expected (effective)} throughput of a query cascade over the temp span. 

We then formulate all the planned queries over all temp spans as the weighted sums of throughputs of individual query throughput over each temp span. 

%\paragraph{$T_{io}(s)$: IO bandwidth when loading a footage from a specific storage tier $s$}
%%To derive the , we drill down to examine the IO throughput on a specific storage tier $s$. 
%The throughput is bound by the lower one between the storage bandwidth and the decoder bandwidth, if decoding is involved. 
%That means:
%\begin{equation}
%T_{io}(s) = \verb!Encoded!(s) ? \min(T_{decoder}, T_{decoded}(s)) : T_{raw}(s)
%\end{equation}

\paragraph{$T_{io}$: IO bandwidth of loading a temp span}
Data in a footage is distributed over multiple storage tiers. 
To obtain this, we first examine $T_{io}(s)$, the average IO bandwidth when loadinDo you have g a footage from a \textit{specific} storage tier $s$
The throughput is bound by the lower one between the storage bandwidth and the decoder bandwidth, if decoding is involved. 
That means:
\begin{equation}
T_{io}(s) = \verb!En!(s) ? \min(T_{decoder}, T_{encoded}(s)) : T_{raw}(s)
\end{equation}

The effective IO over all tiers is bound by the slowest storage tier. \note{explain this more; give more thoughts; how about decoding bw which is shared?}
That is: 
\begin{equation}
T_{io} = \frac{1}{\max_{s \in storage}(D(s) / T_{io}(s))}
\end{equation}

\paragraph{A single operator performance on a footage (a specific temperature $t$)}
%Assume the operator throughput (infinite input bandwidth) is $T_{op}$ and the average IO bandwidth is $T_{io}$.
An operator performance is bound by the lower one between its compute throughput $T_{comp}$ and the aggregated IO throughput $T_{io}$.

\begin{equation}
	T_{op}(t) = min(T_{comp}, T_{io})
\end{equation}
%
%\begin{equation}
%	\begin{aligned}
%	\mathcal{} tput_{hot} 
%	& = w_{hot} \times min (tput_{CV_j}, tput_{I/O_j}) \\
%	\end{aligned}
%\end{equation}
%in which
%\begin{equation}
%	\begin{aligned}
%	tput_{I/O} = 1/max (\frac{t_d}{tput_{DRAM}}, \frac{t_s}{tput_{SSD}},  \frac{t_h}{tput_{HDD}})
%	\end{aligned}
%\end{equation}
%and \note{what does the following mean? the tput when CV consumes data from different storage tiers?}
%\begin{equation}
%tput_{DRAM} = dramen_t \times min(tput_{decode}, tputd_{en}) + dramr_t \times tputd_r
%\end{equation}
%
%\begin{equation}
%tput_{SSD} = ssden_t \times min(tput_{decode}, tputs_{en}) + ssdr_t \times tputs_r
%\end{equation}
%
%\begin{equation}
%tput_{HDD} = hdden_t \times min(tput_{decode}, tputh_{en}) + hddr_t \times tputh_r
%\end{equation}
%Similarly, we have the throughput of querying warm and cold videos.
%
%\begin{equation}
%\begin{aligned}
%\mathcal{} tput_{warm} 
%& = w_{warm} \times min (tput_{CV}, tput_{I/O}) \\
%\end{aligned}
%\end{equation}
%
%\begin{equation}
%\begin{aligned}
%\mathcal{} tput_{cold} 
%& = w_{cold} \times min (tput_{CV}, tput_{I/O}) \\
%\end{aligned}
%\end{equation}
%
%The objective function is the total throughput regarding a specific query, and we need to maximize the objective function.
%\begin{equation}
%	tput = \sum tput_{hot} + tput_{warm} + tput_{cold}\\
%\end{equation}

\paragraph{The performance of a query (as a cascade of operators) on a temp span}
For each operator, it has a probability/distribution of whether triggering it after the previous stages.
For example, when the motion detector detected no motion between consecutive frames, the pipeline will drop the frame and work on further frames.
%We specify the probability that a video chunk triggers the i-th operator as $f_i$.
We specify $f_i$ as the fraction of video chunks (\note{important. the fraction of video time (input frames)}) that trigger the execution all the way until (inclusive) operator $i$. 
The aggregated throughput for consuming this fraction of chunks is bound by operator $i$ which we assume is the slowest one \note{is this correct? also, we implicitly assume serial processing of video chunks}

In the end, the total query performance is determined by the activation frequency of each operator.

\st{the combination of each operators performance} \note{bad wording}.
In all, the total query throughout is
\begin{equation}
\begin{aligned}
\mathcal{} T_{query}(t)
& = \frac{1}{\sum_{i=1}^{n}(f_i \times \frac{1}{T_{op(i)}})} \\
\end{aligned}
\end{equation}


%\paragraph{An operator's weighted throughput on one \istream{} across all temperatures}
%One operator consumes one \istream{} that consists of footages of different temperatures. 
%It is a weighted sum (temperature weights). 
%\begin{equation}
%	T_{op} = \sum_{t \in temp} w(t)  T_{op} (t)
%\end{equation}

\paragraph{All queries weighted throughputs over all temperature spans}
It is a weighted sum (temperature weights) over queries and over temperatures
\begin{equation}
	T_{all} = \sum_{q \in queries} w'(q) \sum_{t \in temp} w(t)  T_{query} (t)
\end{equation}

%\begin{equation}
%\begin{aligned}
%\mathcal{} T_{query}
%& = \frac{1}{time_{query}} \\
%\end{aligned}
%\end{equation}

Since the objective function consists of nested levels of max and min, this is a XXX problem. 

\note{We will validate our model} experimentally in \sect{eval}.
%Suppose we have n operators, and the fraction of the i-th operator is $f_i$, the throughput of i-th CV operator is $tput_{CV_i}$, and the I/O throughput of the i-th operator's resolution is $tput_{I/O_i}$.

%\subsection{Model Applications}
\subsection{Applying the Model}

\textbf{Optimal \istream{} storage policies}
This is equivalent to find model variables (listed in Table XXX) that maximize the global performance utility (9), subject to constraints (1--4). 
\note{what optimization problem is this? Max/min nonlinear? Give a bit more background}
The optimization problem is solved by Python Scipy Optimization \note{less interesting}.

\paragraph{Hardware planner}
Given planned queries and a monetary budget, how do system admins invest \$\$ on hw in order to maximize performance?
We answer this by introducing a cost model atop the performance model.
%
The cost model provides a list of all candidate hardware devices (storage tiers and hardware codec) and their monetary costs. 
The \sys{} planner enumerates all combinations of candidate hardware devices and the associated total cost (as long as the cost is under the budget). 
For each hardware setup, the planner solves the performance model to find the optimal performance utility. 
With the maximized utilities, the planner reports a Pareto frontier: 
each point represents the hardware setup that gives best the performance at that price point. 
We will present detailed hardware planning results in Section XXXX. 



\subsection{Reconfiguration Planning}
As described in \sect{overview}, in response to reconfiguration, \sys{}
updates the optimal storage policies by re-executing the solver. 
To migrate video data across storage tiers with the required codec tasks, 
\sys{} plans a \textit{reconfiguration schedule} to prioritize migration tasks with higher benefits. 
so that the long-running reconfiguration benefits query performance as quickly as possible -- even when the reconfiguration is still in progress. 
%This also allows user to terminate migration at any time while 
This also allows user to preset a fixed time budget (e.g. 2 hours) on migration with the highest performance return. 
Decide new data placement, and determine schedule.
The generic principle is to prioritize migration tasks by their performance reward. 

A reconfiguration mission can be broken down into migration tasks.
We define a migration task as migrating the data chunks from one storage tier on one temperature span \note{should we define it? a sequence?} to the other storage tier. 
For instance, the old policy of a temp span is [20, 20, 60] and the new policy is [10, 30, 60]. 
A migration task is moving half of the chunks on the 1st tier (10\% of total) to the 2nd tier. 
By our definition, within each migration task, the order of moving chunks does not affect the performance goal as they have identical performance impact. 
\note{check}






\note{We assume the performance grows monotonically as migration proceeds. what's the rationale?}
% do we assume something like reserved temp space for swappnig data? 

\paragraph{Problem formulation -- temporal knapsack problem}
$N$ migration tasks, each will use two storage tiers (one inbound, one outbound) and optionally the hardware codec. 
A given migration task $x$ lasts time $T(x)$; the normalized contribution to the overall query performance is $P(x)$. \note{This is always non negative. Why?}
However, $P(x)$ is not always non-negative: adding/removing video streams or hardware resources will make $P(x)$ non-negative; changing user settings result in data exchanging data between fast and slow storage tiers, and will temporarily make $P(x)$ negative. 
To avoid temporary drop, we reserve a small buffer space that can temporarily hold \istream{} that is going to be placed onto slower tiers.
The problem is how to pick unfinished tasks (mapped to storage tiers) to maximize performance contribution \note{improve}. 
Note that: i) 
since we target maximizing performance return and $P(x)$ is ordered, it is always beneficial to execute tasks to completion (without preemption); 
ii) at one given moment, each storage tier serves at most one task (a read or write stream); 
This is because we observed that concurrent read/write streams on storage device result in substantial degradation in total device throughput. \note{need evidences}

Based on the formulation, this is a temporal knapsack problem which is known NP-hard \cite{XXX}. 
Fortunately, we expect the total number of storage tiers is small (e.g. no more than 5), making brutal force (?) solution affordable. 
In a typical three-tier storage (e.g. DRAM, SSD, and HDD), 
the problem can be solved with a greedy approach, as we will explain below. 
%the solution will be further simplified, as we will explain below. 

\paragraph{Solving the migration for 3-tier storage: greedy approach}
Based on our ``no sharing'' observation above, three storage tiers can at most serve one migration task and run it to completion. 
More specifically, let us compare 
i) running one task $x_1$ with the highest return and ii) 
running two tasks $x_2$ $x_3$ (four r/w streams) with lower return concurrently. 
For case ii), one storage tier is inevitably shared by two tasks. 
On this storage tier, the aggregated throughput will be less than serving the $x_2$ or $x_3$ solely. 
The aggregated return is less than serving $x_2$ or $x_3$ solely, which is less than the return of serving $x_1$ solely. 

\textbf{sharing storage tier will degrade (instead of improve) the aggregated storage throughput. This is also because we stream large data chunks. (MB or tens MB)}

\note{put some numbers here.}
is this also true for one read stream and one write stream coming from one tier?


First, \sys{} quantifies the impact of data migration on the short-term performance gain by calculating the score using the following equation. Let $T_{mg}$ be the migration time of the certain task, and the $P_{old}$ and $P_{new}$ be the performance before and after the migration.
	\begin{equation}
		Score = \frac{P_{new} - P_{old}}{T_{mg}}
	\end{equation}
	
\note{performance gain normalized by time?}

Second, \sys{} ranks the tasks by their score in descending order, and the future migration will prioritizes high impacting tasks.
Third, the migration starts from the highest task and launch all the tasks in order.

\note{we will evaluate the produced migration plan ...} \sect{eval}.

\begin{comment}
The choice of the greedy approach stems from the following rationales:
\begin{itemize}
	\item Multiple concurrent read or write streams shares the bandwidth, and always result in lower reward, in that it makes sense to always execute the highest priority stream. \note{Redundant with ii???}
	\item Higher priority tasks is always more beneficial than the combinations of two low-priority tasks.
	\begin{enumerate}[label=\roman*.]
		\item According to pigeonhole principle, we have 3 storage tiers. If we combine two migration tasks concurrently, there are 4 streams coming in or out of one storage tier (one read stream and one write stream for each task). So that there exists one storage tier that is involved in both two migration tasks, and has two concurrent read or write streams.
		\item However, the bandwidth of two read or write streams in parallel will be penalized to $p_1\%$ and $p_2\%$ of the full bandwidth. Normally, 
		\begin{equation}
			p_1\% + p_2\% \leq 1
		\end{equation}
		\note{1. we need to show evidence. 2. IIRC this is also true for one read stream and one write stream coming from one tier, correct?}
		\item Assume the scores for each of the two tasks are $s_1$, $s_2$, and $s$ is the score for the higher priority task. 
		\begin{equation}
			s \geq s_1 \geq s_2
		\end{equation}
		\item The total performance gain for the combination of two low-priority tasks is 
		\begin{equation}
			\begin{aligned}
				\mathcal{} p_1\% \times s_1 + p_2\% \times s_2 
				& \leq (p_1\% + p_2\%) \times s_1 \\
				& \leq s_1 \\
				& \leq s
			\end{aligned}
		\end{equation}
		which is always worse than the performance of the single high-priority task.
	\item
	In conclusion, the high priority single task is always more beneficial than the combinations of two low-priority tasks.
	\end{enumerate}
	\item
	We can extend the combinations of two low-priority tasks to more than two cases, and it does not affect the conclusion we draw out in the upper rationale. 
\end{itemize}
\end{comment}

\iffalse

\note{tiantu's old writeup}

Configuration always adapts to the updates of query profiles and hardware resources. When the user add/remove query profiles, or when the user purchases new hardware devices, e.g., new GPU decoder, or faster storages tiers like DRAM or SSD, the current i-stream configuration is no longer optimized for the highest performance. Hence, \sys{} will rebuild the i-stream and redistribute the data placement. Although large volumes of data migration is costly, \sys{} takes two steps to handle the whole procedure.

\subsection{Model-based Reconfiguration}
With the configuration model provided in section\note{XXX}, \sys{} identifies the new configuration that gives the best query performance.

\subsection{Data Migration}
\sys{} optimizes the data migration by adopting the Greedy Approach in order to benefit query performance as fast as possible -- even when the reconfiguration is still in progress. 
First, \sys{} quantifies the impact of data migration on the short-term performance gain by calculating the score using the following equation. Let $T_{mg}$ be the migration time of the certain task, and the $P_{old}$ and $P_{new}$ be the performance before and after the migration.
	\begin{equation}
		Score = \frac{P_{new} - P_{old}}{T_{mg}}
	\end{equation}
Second, \sys{} ranks the tasks by their score in descending order, and the future migration will prioritizes high impacting tasks.
Third, the migration starts from the highest task and launch all the tasks in order.

The choice of the greedy approach stems from the following rationales:
\begin{itemize}
	\item Multiple concurrent read or write streams shares the bandwidth, and always result in lower reward, in that it makes sense to always execute the highest priority stream. \note{Redundant with ii???}
	\item Higher priority tasks is always more beneficial than the combinations of two low-priority tasks.
	\begin{enumerate}[label=\roman*.]
		\item According to pigeonhole principle, we have 3 storage tiers. If we combine two migration tasks concurrently, there are 4 streams coming in or out of one storage tier (one read stream and one write stream for each task). So that there exists one storage tier that is involved in both two migration tasks, and has two concurrent read or write streams.
		\item However, the bandwidth of two read or write streams in parallel will be penalized to $p_1\%$ and $p_2\%$ of the full bandwidth. Normally, 
		\begin{equation}
			p_1\% + p_2\% \leq 1
		\end{equation}
		\item Assume the scores for each of the two tasks are $s_1$, $s_2$, and $s$ is the score for the higher priority task. 
		\begin{equation}
			s \geq s_1 \geq s_2
		\end{equation}
		\item The total performance gain for the combination of two low-priority tasks is 
		\begin{equation}
			\begin{aligned}
				\mathcal{} p_1\% \times s_1 + p_2\% \times s_2 
				& \leq (p_1\% + p_2\%) \times s_1 \\
				& \leq s_1 \\
				& \leq s
			\end{aligned}
		\end{equation}
		which is always worse than the performance of the single high-priority task.
	\item
	In conclusion, the high priority single task is always more beneficial than the combinations of two low-priority tasks.
	\end{enumerate}
	\item
	We can extend the combinations of two low-priority tasks to more than two cases, and it does not affect the conclusion we draw out in the upper rationale. 
\end{itemize}
\fi


==> planning.tex <==

Based on the XXX tree and storage policies that would be derived, parameterized storage cost model and the given video analytics, the tool presents a set of trade-offs between the monetary investment and analytics performance. 
The admin may choose a best-performing storage configuration under the budget. 
Unlike existing storage planning tools that mostly focus on cloud workloads, our tool factors in the cost of GPU choices (hardware decoders), a major investment which significantly affects throughputs for decoding and CV cascade. 
%places the resultant partitions in heterogeneous storage tiers, and dynamically migrates the video data across storage tiers.

==> runtime.tex <==
% !TeX root = main.tex

%\section{Runtime Support}
\section{Runtime Scheduling}
\label{sec:runtime}

The \sys{} runtime provides three services: 
\begin{itemize}
\item Ingestion: ingesting video streams sent from cameras; 
\item Retrieval: loading \istream{} (footage) in response to query execution; 
\item Migration: moving data across storage tiers for reconfiguration (and for data aging). 
\end{itemize}

For the three services \sys{} executes a set of primitive tasks, including db operation (store, load, and delete); and codec operation (decoding and transcoding). 
Despite our modeling/planning optimizes for the case when one query or reconfiguration runs alone, \sys{} supports co-execution of three services. 
\sys{} schedules them to minimize interference. 
To do so it provides two core mechanisms. 

\subsection{Scheduling for heterogeneous services}
\sys{} continuously admits primitive tasks and executes them on its db and codec backends. 
The three services have disparate performance demands (QoS): 
ingestion needs to keep pace with the incoming video data streams (the input buffer for containing unprocessed data must be under certain threshold); 
retrieval needs to return data as soon as possible (actual data load is as soon as possible; speculative or prefetch can be best effort); 
migration is latency sensitive for query addition, and best effort for performance optimization. 

\subsection{Key ideas}
While serving multiple services, \sys{} strives to achieve a set of objectives. 

\begin{itemize}
\item Respect (trade off among) service QoS requirements. For instance, do best effort to catch up with ingestion streams. 
\item Even progress across multiple istreams. This is important one query consumes multiple i-streams (note that it may consume only selected chunks from one i-stream as being triggered by earlier operators). 
The query progresses only when it receives all the requested video chunks earlier than certain video time $t$, which enables it to assert all data prior to $t$ has been completed and processed. 
The same idea applies to ingestion (although less urgent). 
\item Fairness among multiple invocations of the same service.  \note{less important?}
\end{itemize}

Without our design, the \sys{} lacks notion of importance of primitive tasks and is unable to schedule them properly.

Goal: matches the IO throughput with the CV throughput, but not exceed that which leads to excessive in-memory buffering. 
Then use the remaining IO bandwidth serving other services. 

\subsection{Key mechanism}

Our key mechanism is tasks tagged with i-streams (for scheduling). 
the properties of services are propagated to i-streams and then tasks. 

\st{For each resource (storage tier and codec), \sys{} maintains multiple (a hierarchy of queues).}
One class (level) is for one service;
in the class, one queue holds all requests coming one \istream{}.

Define: a device as a storage tier or a codec. 

\sys{} embodies a unified scheduler for all incoming requests. 

The scheduler keeps ``outstanding requests'' sent to all devices but not completed yet. 
It strives to maintain a certain number of outstanding requests at each devices to keep all devices busy. 
The scheduler is invoked (driven) by i) arrival of new requests and ii) completion notification of requests from devices. 
When outstanding request at a certain device drop below a threshold, the scheduler examines all the requests it has received so far and tries to identify a batch (to amortize overhead) to dispatch to the particular device. 

\begin{itemize}
\item 
The highest priority is ingestion (avoid data loss). The scheduler first checks if it can catch up with the ingestion. For instance, if the ingestion buffer exceeds a threshold. If so, it dispatches pending ingestion requests to db/codec until the ingestion buffer usage is low enough. \note{improve}

\item 
For retrieval: the scheduler tracks the \textit{progress} watermarks of all istreams (queries?). 
For each query, it identifies the one with lowest watermark (i.e. the most lagged istream) and pauses serving istreams of which watermarks are too far ahead (i.e. excluding their requests from consideration). 
The rationale is that the whole query will not make progress until the most lagged istream catches up. 
The scheduler dispatches the identified requests to storage/codec -- if any, dispatch them. 

\item 
If no requests are dispatched to a device in this round, the scheduler considers migration requests. 

\end{itemize}

\st{
\sys{} assigns such priority levels (QoS classes) to services. 
\sys{} tags the primitive tasks with the service QoS classes. 
It then embodies a hierarchy scheduler for each resource (a task primitive queue at each resource): db at each storage tier, and codec. 
Across different QoS classes, it uses priority scheduling (always giving preference to high QoS classes). 
Within each QoS class, it uses round robin among services to ensure fairness. 
It runs each task primitive over a data chunk to completion. }


\textbf{Notion: progress/watermark -- schedule based on the progress instead of at individual tasks}

By doing so, \sys{} exploits parallelism among hardware devices. 


\Paragraph{Scheduling and optimizing i-stream flows}
\sys{} orchestrates tasks of IO, decoding, and data move. 

\begin{itemize}
\item 
It prioritizes tasks belonging to different workloads. 
query -- IO and decoding (high throughput)
data ingestion -- IO and transcoding (low throughput, realtime)
data aging (migrate across storage tiers) -- IO (low throughput, background)
reconfiguration -- IO and transcoding (high throughput)

\item 
For i-stream flows serving an active query, it ensures all i-streams to flow with even progress in video time, despite that these i-streams come from tiers with different IO throughput, have different data rates, and incur different decoding overhead. 
The framework tracks a key notion -- video watermark -- for all involved i-streams and as they are loaded, decoded, and joined.
By tracking video watermarks, \sys{} matches the progresses of all i-streams with the CV's progress. 
By doing so, it maximizes the efficient use of memory by avoiding excessive buffering. 

The watermark notion applies to ingestion and retrieval. 

\item 
Since the throughput is high, \sys{} ensures the data path is efficient. 
It maximizes zero copy. It maximizes parallelism among data load, decoding, and move. 
\end{itemize}

Other contributions?
\begin{itemize}
\item buffers
\item data/decoding parallelism 
\item ???
\end{itemize}

\note{prefetch -- move somewhere?}
Depending on the storage policy of an \istream{}, chunks of the \istream{} either encompass raw or encoded video data. 
i) for maximum parallelism, \sys{} should be able to encode/decode individual chunks separately. 
This requires chunk boundary to be at least ...
(i-frame separation, GOP...). 
ii) 
During query execution, the \sys{} prefetchs the chunks ahead of the analytics consumers into memory buffers. 
The prefetcher loads data chunks from multiple tiers concurrently to exploit parallelism between tiers. 
The prefetch window must contain chunks from multiple tiers simultaneously to smooth out the IO throughput spikes. 
otherwise: one chunk from SSD -- to fast; one chunk from HDD -- to slow. 


\subsection{Prioritize primitive tasks}
For \sys{}, three runtime services could be further segmented into multiple primitive tasks with both disk and codec operation.
\begin{itemize}
	\item Ingestion: store, decode+store
	\item Retrieval: load
	\item Migration: load+store, load+decode+store, load+encode+store
\end{itemize}
Given above primitive tasks, \sys{} could schedule these tasks based on their priority.
Assume $P$ represents the priority of a single primitive task.
Further, for a specific primitive task, there are three metrics to evaluate its priority level: service type, device idleness, and request arrival order.
\begin{equation}
	P = T_s \times W_{service} + T_r \times W_{resource} - t,
\end{equation}
In above definition, the weights of each metric is defined to leverage the importance of each metric.
\begin{equation}
	W_{Service} \gg W_{Resource}
\end{equation}
$T_s$ is the rank of three types of services.
\begin{equation}
	T_s \in  \{1=\text{migration},
	2 = \text{retrieval},
	3 = \text{ingestion}\}
\end{equation}
$T_r$ indicates the idleness of original/destination device.
It tries to balance the device usage and avoid device idleness, but its impact never exceeds the priority of service type.
\begin{equation}
	T_r \in \{0 = \text{device busy}, 1=\text{device idle}\}
\end{equation}
$t$ represents the chronological arrival order of each task.
Tasks with smaller $t$ indicates earlier arrival, thus will have relatively larger priority $P$.
\begin{equation}
	t \in (0, max), t\in N
\end{equation}
With the above definition of priority, the scheduler will pick up the next primitive task with the largest $P$.

==> tab-fc.tex <==
% !TeX root = main.tex

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
%\footnotesize
\centering
%\caption{Definitions}
\caption{Knobs and their possible values considered in this work. 
Total: XX knobs and XXX (100?) options}
\label{tab:videoset}
%\vspace*{-1em}

\begin{tabular}{ll}
\textbf{Accuracy} & \textbf{Operator 1}          \\
L1  \\ (24)
L2    \\
L3      \\
L4 \\
\end{tabular}

	
%\vspace*{-2em}
\end{table}

==> tab-resource.tex <==
% !TeX root = main.tex

\begin{table}[]
%\footnotesize
\centering
%\caption{Definitions}
\caption{A video store's major components and hardware resources used by them XXX combine with fig 2 XXXX}
\label{tab:resource}
%\vspace*{-1em}

%\begin{tabular}{ll}
%Components    &                      Hardware resources       			\\
%Ingestion   & Coding throughput (saving as encoded) or disk throughput (saving as raw)   \\
%Storage     & Disk capacity               			\\
%Retrieval   & Hw decoder (built-in GPU) and disk bandwidth   \\
%Consumption & CPU time or GPU time for executing op 
%\end{tabular}

\includegraphics[width=.95\linewidth]{figs/platform2}
	
%\vspace*{-2em}
\end{table}


==> tab-videoset.tex <==
% !TeX root = main.tex

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
%\footnotesize
%\centering
%\caption{Definitions}
\caption{The video datasets used in our evaluation. They are captured from live camera streams}
\label{tab:videoset}
%\vspace*{-1em}

\begin{tabular}{{|c|c|}}
	\hline
	\textbf{Video Datasets} & \textbf{Description}   \\
	 \hline
	 \textit{dash-cam} & A dash camera in a parking lot  \\
		\hline
	 \textit{park} & A surveillance camera in a parking lot  \\
	 \hline
	 \textit{airport} & JAC parking lot live camera   \\
	 \hline
	 \textit{jackson} & Jackson Town Square live camera\\
	 \hline
	 \textit{miami} & Miami Beach crosswalk live camera\\
	 \hline
	 \textit{tucson} & Tucson 4-th avenue live camera \\
	 \hline
\end{tabular}
\vspace*{-10pt}
\end{table}

==> table-variables.tex <==
% !TeX root = main.tex

\begin{table}[t!]
\centering
%\includegraphics[width=0.45\textwidth{}]{./figs/benchmarks} 
\begin{center}
	\centering
	\begin{tabular}
		{ | m{4.8em}<{\centering} | m{6.15cm}<{\centering}|} 
		%{|c|c|}
		\hline
		\centering \textbf{Term} &   \textbf{Description} \\ 
		\hline
	\end{tabular}
	\begin{tabular}
		{ | m{4.8em} | m{6.15cm}|} 
		
%		\multicolumn{2}{|c|}{\textbf{Hardware Specifications -- Global}}  \\
%		\hline
%		$T_{decoder}(i)$ & Decoder throughput for the fidelity chosen by operator $i$\\
%		\hline
%		$T_{trans}(i)$ & Transcoding throughput for the fidelity chosen by operator $i$\\
%		\hline
		
		
		\multicolumn{2}{|c|}{\textbf{Storage specifications -- for Storage tier $s$}}  \\
		\hline		
		$T_{encoded}(s)$ & Read throughput of encoded chunks \\
		\hline
		$T_{raw}(s)$ & Read throughput of raw frames (in bps)\\
		\hline
		$W(s)$ & Disk write speed of tier $s$ (in bps)\\
		\hline
		$C_{s}$ & Disk capacity of tier $s$ \\
		\hline
		
		\multicolumn{2}{|c|}{\textbf{Analytics Profiles -- for an operator $i$}}  \\
		\hline
		$f(i)$ & Activation frequency of the i-th operator (in its enclosing query) \\		
		\hline		
		$B_{r}(i)$ & Raw bitrate of i-th stage fidelity video \\ 
		\hline
		$B_{e}(i)$ & Encoded bitrate of i-th stage fidelity video \\ 
%		\hline
%		$N_{cam}$ & number of ingested streams from the camera\\ 
		\hline
		$T_{decoder}(i)$ & Decoder throughput for the fidelity chosen by operator $i$\\
		\hline
		$T_{trans}(i)$ & Transcoding throughput for the fidelity chosen by operator $i$\\
		\hline

		
		\multicolumn{2}{|c|}{\textbf{User settings -- global}}  \\
		\hline
		$N_{cam}$ & number of ingested streams from the camera\\ 		
		\hline
		$fps$ & fps of the ingestion video \\
		\hline
		$L_t$ & Time length of data temperature $t$ \\ 		
		\hline
				
		\multicolumn{2}{|c|}{\textbf{User-set weights}}  \\
		\hline
		$w'$ & Weight of queries \\ 		
		\hline
		$w$ & Weights of different temperatures \\ 
		\hline
		\st{$S(i, t)$} & \note{derived from above}. Video size with fidelity chosen by operator $i$ and temperature $t$ \\
		\hline
		
		
				
		\multicolumn{2}{|c|}{\textbf{Storage policies -- to be solved}}  \\
		\hline
		\verb!En!(i, s, t) & Encoded video footages for operator $i$ on tier $s$ under temperature $t$? \\
		\hline
		$D_t(i, s)$  & Fraction of the data stored on tier $s$ under temperature $t$ for operator $i$\\ 
		\hline
		
		\multicolumn{2}{|c|}{\textbf{Objectives (?)}}  \\
		\hline		
		$T_{io}$  & IO bandwidth when loading a footage from all storage tiers\\ 
		\hline
		$T_{op}$ & Throughput of a single operator\\
		\hline
		$T_{comp}$ & Computation throughput of the operator \note{discuss with Tiantu}\\
		\hline
		$T_{query}$ & Operator's weighted throughput  \\
		\hline
	\end{tabular}
\end{center}
%\vspace{-10pt}		% use as needed
\caption{Model Variables with $T$ -- \textbf{all throughput/bandwidth in frames per second. Do we need to mention query??}}
\label{tab:benchmarks}
%\vspace{-20pt}		% use as needed
\end{table}


==> todo.tex <==
% !TeX root = main.tex

\textbf{TODO:}

%\note{argument: early operators already load the video. no need to load again for later operator}

\note{Storage is cheaper than compute. The storage hardware designed for video surveillance (write-most workloads) is blooming. 
The per-GB cost keeps dropping. }

%\note{motiv exp: which hw we use?}

%\note{2D search problem}
%\note{different image quality changes the search path on each 2d plane. will that give us different set of Rconsume? (even lower Rconsume?)}


%\textbf{Robust to opp cost variation}
%erosion plan? Do we need to frequently update the plan?

%\note{clarify we don't consider the knob that affects image}


%\note{fig multi option}
%	((XXX (d) --> frame sampling for NN) XXX )
%	Mention monotonic impacts? Not impact consumption??
		
